Detection of WIMP-like dark matter in some extensions of the Standard Model

One of the most popular classes of candidates for dark matter are Weakly Interacting Massive Particles (WIMPs), i.e. particles possessing masses and couplings falling roughly within the electroweak scale. Apart from offering a natural mechanism for explaining dark matter, WIMPs also provide us with a hope that they could be detected through their non-gravitational interactions. In such an eventuality, we shall certainly get closer to the goal of identifying the true nature of dark matter. After introducing some formalism and elements of theory, we study the phenomenology of WIMP-type dark matter both in a model-independent manner as well as in the framework of specific models, focusing on the prospects for detection in running or oncoming direct and indirect detection experiments.

==> susy/LightHiggs.tex <==
\section{The Light Higgs Scenario}
The BMSSM framework discussed in the previous section tries to alleviate the little
hierarchy problem by invoking new physics inducing a positive contribution to the
higgs mass. However, in section \ref{LittleHierarchyProblem} we discussed another
possible way out.

As we saw in eq.\eqref{HiggsProdLEP}, the higgs production cross-sections for the channels favoured at LEP2 
depend not only on its mass, but also on its couplings. In particular, we saw that the $hZZ$
coupling receives a $\sin(\beta - \alpha)$ suppression with respect to the Standard Model 
one. If  $\sin(\beta - \alpha) < 1$, then the LEP bound
could potentially be evaded (or, more precisely, modified towards lower masses).
The problem in CMSSM models arose from the fact that typically $\sin(\beta - \alpha) \sim 1$, 
a regime which is usually called the \textit{decoupling regime}, since the pseudoscalar higgs is much
heavier than the lightest $CP$ - even higgs boson.

Departing from the mSUGRA/CMSSM framework allows to open a parameter space where the $114.4$ GeV
limit on the higgs mass no longer holds, due to the decrease in the $hZZ$ coupling. In this regime,
all higgs bosons can have comparable masses, hence it is often called the \textit{non-decoupling zone}.
The masses of the neutral higgses can reach down to the value of the $Z$ boson \cite{Djouadi:2005gj}
without conflicting the LEP2 constraints. Interestingly, such a LHS with $m_h \sim 98$ GeV can 
apparently also accomodate the $2.3 \sigma$ LEP2 excess \cite{Barate:2003sz}. The little hierarchy
problem is concretely evaded due to the fact that since the higgs mass can now be much lower than
the LEP2 conventional limit, radiative corrections need not be large and hence the assumptions on
the stop sector can be rendered less restrictive.

Several approaches towards the possibility for a light higgs have been examined in the
literature \cite{Kane:2004tk, Kim:2006mb, Belyaev:2006rf, Chattopadhyay:2008hk, Bhattacharya:2009ij}.
One such framework is a non-universal higgs mass (NUHM) model \cite{Chattopadhyay:2008hk, Bhattacharya:2009ij}
where the Higgs masses are attributed different values than the other scalars at the GUT scale.
Assuming such a condition does by no means necessarily abandon Grand Unification. On the 
contrary, the Higgs bosons often live in different representations of GUTs and can therefore
acquire different masses.

Describing the full phenomenology of such a framework goes beyond the scope of the present work.
We shall focus on the analysis performed in \cite{}, where we examined a particular variant of 
a NUHM model and its dark-matter related phenomenology.

\subsection{The model and its constraints}
The Light Higgs Scenario can be realized by slightly relaxing the constraints of the CMSSM. In particular,
if one assumes non-universal higgs masses at the GUT scale, then it turns out possible to obtain 
viable models which yield masses lower than $114.4$ GeV, without violating the LEP2 bounds, through the
reduction of the $\sin(\beta - \alpha)$ coefficient.
The model can be described by seven parameters
\begin{equation}
 m_{1/2}, \ A_0,  \ \mbox{sign}(\mu), \ \tan\beta, \ m_0, \ m_{H_u}^2, \  m_{H_d}^2
\end{equation}
where the GUT-scale common scalar mass $m_0$ concerns all scalars but the two Higgs bosons.

Starting from this set of parameters it is possible to retrieve the low-energy quantities  
as well as a viable parameter space passing all electroweak constraints. $\mu$ and $m_A$
can be computed using the Renormalization Groups Equations as well as the requirement
for radiative EWSB, through the following equations
\begin{eqnarray}
 \mu^2 & = &
-\frac{1}{2} M^2_Z +\frac {m_{H_D}^2-m_{H_U}^2 \tan^2\beta} {\tan^2\beta -1}
+ \frac {\Sigma_1 -\Sigma_2 \tan^2\beta} {\tan^2\beta -1}\\
\sin2\beta & = & 2B\mu/(m_{H_D}^2+m_{H_U}^2+2\mu^2+\Sigma_1+\Sigma_2)\\
m_A^2 & = & m_{H_D}^2+m_{H_U}^2 +2\mu^2 \sim m_{H_D}^2-m_{H_U}^2
\label{mumA}
\end{eqnarray}
where $\Sigma_i$'s represent the one-loop radiative corrections \cite{Arnowitt:1992qp, Gamberini:1989jw, Barger:1993gh}
and the last of the three equations holds at tree-level given that one can approximate 
$\mu^2 \sim -m_{H_U}^2$ for $\tan\beta \ge 5$. All the EW scale parameters and masses
are computed using the SuSpect package \cite{Djouadi:2002ze}.

Then, a set of electroweak observable constraints can be imposed in order to produce realistic
models:
\begin{itemize}
\item {{\bf Higgs boson mass limit:}} 
In the non-decoupling 
region when $m_A$
becomes very light so that one has $m_A \sim m_H \sim m_h \sim M_Z$ 
the lower limit of $m_h$ goes down to 93 GeV or even lower\cite{Barate:2003sz}. 
We define the \textit{light Higgs boson scenario} by demanding that 
$\sin(\beta-\alpha)^2~<~0.3$ (or $\sin(\beta-\alpha)~<~0.55$) and at the same
time $93<m_h<114$. In practice, we slightly relax the limit on $\sin(\beta - \alpha)$
and demand $\sin(\beta-\alpha)~<~0.6$. An interesting feature is that in this case, the
LEP2 limit of roughly $114$ GeV now starts to apply for the heavier higgs boson, since its
coupling for the higgstrahlung process is $g_{zzH} \propto \cos(\beta-\alpha)$, which
now becomes dominant. So, in order to obtain an acceptable
SUSY spectrum with $93<m_h<114$, in addition to the desired 
value for $\sin(\beta-\alpha)$, one also requires $m_H>114~$GeV. 

On the other hand, in the decoupling region 
($\sin(\beta-\alpha) \sim 1$ ), the $m_h \gtrsim 114$ GeV limit 
needs to be respected. 
However we note that there is an uncertainty of about 3~GeV
in computing the mass of the light Higgs boson
\cite{Heinemeyer:2004gx, Heinemeyer:2004kg, Degrassi:2002fi, Allanach:2004rh}. This
theoretical uncertainty primarily originates from momentum-independent
as well as momentum-dependent two-loop corrections and higher loop corrections
from the top-stop sector. Consequently, a lower limit of $111$~GeV is often 
accepted for the SUSY light Higgs boson mass $m_h$.  
 

\item {\bf $Br(b\rightarrow s\gamma)$ constraint:} 
In models like mSUGRA, 
the most significant contributions to $b\rightarrow s\gamma$ 
originate from charged Higgs and chargino exchange diagrams.
The charged Higgs 
($H^- - t$ loop) contribution has the same sign and comparable strength 
with respect to the $W^- - t$ loop contribution of the SM, which already 
saturates the experimental result. Hence, in scenarios where the charged Higgs mass
can be very small, satisfying the $b \rightarrow s \gamma$ constraint requires 
a cancellation between the two diagrams.  
This in turn requires a particular sign of $\mu $ or 
more precisely, that $\mu$ and $A_t$ are of opposite sign. The effect
of this constraint on the Light Higgs boson zone has been discussed
in \cite{Kim:2006mb}.  We have 
used the following
 3$\sigma$ level constraint from $b \rightarrow s \gamma $ with 
the following limits\cite{Koppenburg:2004fz, Aubert:2002pd, Barberio:2006bi}. 
\begin{equation}
2.77 \times 10^{-4} < Br (b \rightarrow s \gamma) < 4.33 \times 10^{-4}.
\label{bsgammalimits}
\end{equation}
\item {\bf $Br(B_s\rightarrow \mu^+ \mu^-)$ constraint:} 
Similarly, the flavor physics observable 
$B_s\rightarrow \mu^+ \mu^-$ may become very significant in 
this particular parameter space. The current experimental limit 
for $Br(B_s \to \mu^+ \mu^-)$ 
coming from CDF\cite{Aaltonen:2007kv} can be written as (at ${\rm 95\,\%\,C.L.}$) 
\begin{eqnarray}
{\rm Br} ( B_s \to \mu^+ \mu^-) < 5.8 \times 10^{-8}. 
\label{Bsmumu}
\end{eqnarray}
The estimate of 
$ B_s \to \mu^+ \mu^- $ in the MSSM depends strongly
on the mass of the A-boson and on the value of $\tan \beta$. In particular, the  
neutral Higgs boson contribution scales as $ m_A^{-4}$ whereas 
there is an additional dependence on $(\tan \beta)^6$. However, in the
present analysis, we choose $\tan\beta~=~10$ which makes this constraint
less restrictive for most of the parameter space.
\item {\bf WMAP constraint :}
In computing the relic density constraint, we consider 
the following 3$\sigma$ limit of the WMAP data\cite{Dunkley:2008ie}, 
\begin{equation}
0.091 < \Omega_{CDM}h^2 < 0.128.
\label{relicdensity}
\end{equation}
Here $\Omega_{CDM}h^2$ is the dark matter 
relic density in units of the critical
density and $h=0.71\pm0.026$ is the Hubble constant in units of
$100 \ \rm Km \ \rm s^{-1}\ \rm Mpc^{-1}$. We have used the 
code Micromegas\cite{Belanger:2008sj} for 
computing the neutralino relic density.

\end{itemize}

\section{Dark matter in a LHS with Non - Universal Higgs Masses}

\subsection{Relic density and electroweak observables}
The first step in our analysis is to impose the various constraints as explained before
and compute the regions where the WMAP bounds are satisfied.
Our main results are presented in Figs.\ref{a01100} and \ref{a01000}. In both cases,
we depict the parameter space points consistent with the WMAP data in the 
$m_{1/2}-m_A$ plane (red dots), while assuming a moderate value for $\tan\beta=10$. 

Let us first concentrate on figure \ref{a01100}. 
The other parameters are set at $m_0=600~$ GeV, $A_0=-1100$ GeV. We have 
varied the mass parameters $m_{H_u}$ and $m_{H_d}$ in the regions 
$0 < m_{h_u}^2 < m_0^2$ and $-1.5 m_0^2 < m_{h_d}^2 < -0.5 m_0^2$ so as
to obtain $\mu$ and $m_A$ parameter values in the desired range. 
%within $0<\mhu<m_0^2$ and $-1.5 m_0^2<\mhd<-0.5 m_0^2$. 
This provides us with
reasonably large values of the $\mu$ parameter for the valid parameter points.
The lightest neutralino is mostly $\tilde B$ - like 
(although with a non negligible $\tilde H$ component).

In the same plot, we also show contours for the lightest Higgs mass ($m_h$) and
$\sin(\beta-\alpha)$. All the parameter space points with $\sin(\beta-\alpha)< 0.6$
are characterised, according to our conventions, as belonging to the  Light Higgs boson scenario,  
where the Higgs mass can evade the LEP2 limit due to
the reduced coupling with the $Z$ boson. On the other hand, admitting 
a 3 GeV uncertainty in the Higgs mass calculation, as mentioned, we delineate
the regions corresponding to 111 GeV < mh < 114 GeV. Satisfying WMAP for smaller $m_{1/2}$ values, 
imposes lighter squarks as well as lighter gluinos.
\\
There are two distinct regions in the parameter space satisfying the 
relic abundance constraint:

\begin{itemize}
 \item The light Higgs pole annihilation region where
 neutralino annihilation 
produces an acceptable relic density via
the $s$ - channel exchange of a light Higgs. This
region extends in the direction parallel to the $m_A$ axis with gaugino mass 
value $\sim 140$ GeV.
In plain mSUGRA models, this zone is highly restricted due to 
flavor physics constraints \cite{Djouadi:2005dz,Chattopadhyay:2010vp}. 
The spin independent cross-sections\cite{Chattopadhyay:2010vp},
on the other hand, could reach the CDMS-II\cite{Ahmed:2009zw} result.

 \item The second region which is also a funnel region, but now
annihilations are principally due to $s$ - channel exchange of $A$ and $H$ bosons, 
since now $2m_{\tilde \chi_1^0} \simeq m_A, m_H$. 
Similar to the case of mSUGRA, this WMAP - satisfying
region in the NUHM model is principally characterized by the pseudoscalar 
Higgs boson -  mediated resonant annihilation.  The exact or near-exact 
resonance regions have very large annihilation cross-sections resulting in  
under-abundance of dark matter. In fact, an acceptable relic density
can be produced when the $A$-width is 
quite large and $2m_{\tilde \chi_1^0}$ can be appreciably away from the exact 
resonance zone. This is precisely the reason for the two branches of red circles 
that extend along the direction of $m_{1/2}$ in figure \ref{a01100}. The same
effect was present also in the $h$ - pole region in our BMSSM analysis.
\end{itemize}

Since we wish to focus on the LHS scenario, of particular interest
is the region where $\sin(\beta-\alpha)< 0.6$. 
In this regime, the lightest neutralino is characterized by a quite small
mass, $55<m_{\chi^0_1}<65$ GeV, whereas the $A$ boson plays a dominant role 
in the annihilation process. Now, apart from the mass of the $A$ bosons, 
neutralino pair annihilation also depends on the coupling 
${\cal{C}}_{\chi_1^0 \chi_1^0 A} \sim N_{11} N_{13}$. 
We recall that the Higgsino component $N_{13}$ of the LSP
is essentially determined by the $\mu$ parameter. With a relatively large $\mu$
parameter, thus smaller Higgsino components as in this case, 
satisfying the relic density constraint in the non-decoupling
region of the Higgs boson requires much 
smaller neutralino masses $\sim 55-65$ GeV. In other words, the neutralino 
in this case cannot be too far from the exact resonance condition.
In this respect, as the neutralino mass increases, the WMAP-compliant
regions extend in the direction of larger $m_A$.
However then the Higgs bosons fall into the other category, i.e. in the decoupling
region. Interestingly, even this WMAP - satisfying zone does not require
large values for gaugino masses. We shall followingly see that this whole region
can lead to large gamma-ray as well as antiproton signals in present or oncoming
experiments.
\\ \\
Before presenting our results on indirect detection, we should
also discuss the flavor physics observables $b \rightarrow
s \gamma$ and $B_s \rightarrow \mu^+ \mu^-$. Since we choose a rather 
moderate value for $\tan\beta$($=10$), the $B_s \rightarrow \mu^+ \mu^-$ constraint is 
not very stringent for the parameter space as shown in Fig.\ref{a01100}.
On the other hand $Br(b \rightarrow s \gamma)$ constitutes a strong
constraint particularly in the non-decoupling region 
where charged Higgs bosons could be very light. However, 
for large negative $A_0$ values, hence negative values of $A_0$ at the EW scale, 
one of the stop eigenstates
becomes lighter due to large mixing and this provides a cancellation
between charged Higgs and chargino - induced diagrams. Choosing $A_0=-1100~$GeV 
at $M_{GUT}$, almost all parameter space points and more importantly the whole WMAP
allowed region in the $m_{1/2}-m_A$ plane can satisfy the constraint. 
\\ \\
Fig.\ref{a01100} also contains some gray zones, which correspond to some further
constraints:\\
 (i)For $m_{1/2} \ge 140~$ GeV, parameter space points with
$m_A$ smaller than roughly $100~$GeV 
are not compatible with the Higgs mass limit in the non-decoupling zone i.e,
here one has $m_h<93~$GeV.\\ 
 (ii) For $m_{1/2} \le 140~$GeV, the gluino becomes 
lighter (we demand $m_{\tilde g}> 390~$GeV for a valid parameter space point\cite{Amsler:2008zzb}) and
then very soon the chargino becomes too light with $m_{\chi_1^\pm}<103.5~$GeV. We should
note here that a light Higgs  with mass $m_h\le 93~$ GeV may be allowed,
but then $\sin(\beta-\alpha)$ needs to be further suppressed. However this
region is then further constrained and we do not consider it here. 

It should be noted that for this first scenario, the parameter value choice 
of fig.\ref{a01100} yields relatively light neutralinos, of masses up to $65$ GeV.
\\ \\  
Next, we probe a parameter space region where neutralinos become heavier, remaining
nevertheless in the {\it Light Higgs boson} zone. Once again, the relic density constraint 
is satisfied by $s$ - channel resonnant $A$ exchange. 
For illustration we fix $m_0$ at a very similar value as previously, 
i.e $m_0=600~$GeV while the trilinear coupling $A_0$ is fixed at
$A_0=-1000$ GeV in order to make $b \rightarrow s \gamma$ less restrictive.  
Then, as before,
$m_{H_u}^2$ is set to $2.4 m_0^2$ and $m_{H_d}$ is varied in the region
$-0.3 m_0^2 < m_{H_d}^2 < 0$. These choices yield small values for the $\mu$
parameter ($150<\mu<300$), hence the LSP can have a significatn higgsino component.

The corresponding results can be seen in fig.\ref{a01000}.
It can be seen that 
$m_{1/2} \sim 300~$ correspons to the non-decoupling zone for the Higgs boson.
Clearly, the lightest neutralino($m_{\tilde \chi_1^0} \sim 120~$GeV) 
is quite far from the resonant annihilation
condition i.e. the so-called $2m_{\tilde \chi_1^0} \simeq m_A$. In comparison 
to the previous case, where the $b \bar{b}$ final state has the maximum branching
ratio, here several other final states involving the Higgs bosons ($Zh, 
ZH, W^\pm H^\pm, hA, HA, hh$) open up. We should note that
$m_{\tilde \chi_1^0}$ cannot too large as then the neutralino would be 
even further away from the resonance condition, which in its turn makes the pair
annihilation via $A$-boson exchange less efficient. As in the previous scenario, 
the $b \rightarrow s \gamma$ constraint does not influence the WMAP - compliant 
zones. The gray areas correspond to the same constraints as before.

\label{results}
\begin{figure}[ht!]
\begin{center}
\includegraphics[width=12cm,height = 10cm]{./susy/mhalf-ma_neg1100.eps}\\
\end{center}
\caption{{\footnotesize
WMAP - compliant parameter space points (red dots) in the $m_{1/2}-m_A$ plane. 
The correct relic density is obtained via $s-$channel $h$ 
or $A,H$ exchange annihilations. Neutralino masses with $m_\chi \sim 55-65$ GeV 
correspond to the light Higgs boson region. Detectability of the
photon and anti-proton signals are represented by $D^{\gamma}$ and $D^{\bar{p}}_{MED}$. 
The complete $A$ pole annihilation region is within the reach of the Fermi and 
upcoming AMS-02 experiments. All mass parameters are in GeV.
}}
\label{a01100}
\end{figure}

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=12cm,height = 10cm]{./susy/mhalf-ma_neg1TeV.eps}\\
\end{center}
\caption{{\footnotesize
Same as Fig.\ref{a01100}, except the light Higgs boson zone
is shifted to larger gaugino mass values. 
As before, all mass parameters are in GeV.
}}
\label{a01000}
\end{figure}


\subsection{Indirect detection in the NUHM model}
The next step is to compute constraints from  and perspectives for dark matter detection experiments.
This shall be done for gamma-rays coming from DM annihilation at intermediate galactic latitudes and
for the Fermi mission, as well as antiprotons at the PAMELA and AMS02 experiments.

We ommit the relevant study for positrons, since the previous two model examples in this work 
reveal rather pessimistic perspectives for this channel.

Before proceeeding with the analysis, it is again useful
to define the measure, in particular what we mean by ``exclusion''
and ``detectability''.
Let's denote by $N_{\mbox{\begin{tiny}DM\end{tiny}}}$ the theoretical number of gamma-rays or antiprotons within
one energy bin, $N_{\mbox{\begin{tiny}bkg\end{tiny}}}^{\mbox{\begin{tiny}Th\end{tiny}}}$ the
theoretical number of events coming from background sources, 
$N^{\mbox{\begin{tiny}Exp\end{tiny}}}$ the mean experimental number of events in the same bin, 
$\sigma^{\mbox{\begin{tiny}Exp\end{tiny}}}$ the experimental error in this number as given by the
Fermi or the PAMELA collaboration and $\sigma^{\mbox{\begin{tiny}Stat\end{tiny}}}$ the naive statistical error
expected which, for a given background model is actually equal to 
$\sqrt{N_{\mbox{\begin{tiny}bkg\end{tiny}}}^{\mbox{\begin{tiny}Th\end{tiny}}}}$ assuming gaussian
statistics.

Then, we shall be calling a parameter space point ``$3-\sigma$ excluded'' if even in a single bin
it satisfies the condition:
\begin{equation}
 N_{\mbox{\begin{tiny}DM\end{tiny}}} + N_{\mbox{\begin{tiny}bkg\end{tiny}}}^{\mbox{\begin{tiny}Th\end{tiny}}} > 
N^{\mbox{\begin{tiny}Exp\end{tiny}}} + 3 \sigma^{\mbox{\begin{tiny}Exp\end{tiny}}} .
\label{exclusion}
\end{equation}
That is, a parameter space point shall be considered as excluded if the sum of the background-predicted
flux (the fact that it is actually a post-diction does not alter the reasoning) and the DM-induced one
becomes larger than the 3-$\sigma$ upper limit of the observed flux.

On the other hand, we shall be calling a parameter space point ``$3-\sigma$ detectable'' if even
in a single bin, it satisfies the condition
\begin{equation}
 N_{\mbox{\begin{tiny}DM\end{tiny}}} > 3 \sigma^{\mbox{\begin{tiny}Stat\end{tiny}}}
\label{detectabilityCriterion}
\end{equation}
i.e. if our DM candidate produces a signal which is larger than a $3\sigma$ statistical fluctuation
of the background. In this case, we shall consider that the candidate should be able to produce a 
significant excess so as to be observed. 
Obviously, the former results shall be subject to severe changes according to
deviations from gaussian statistics, further experimental errors, systematics etc.
More detailed analyses are obviously performed within the experimentalist community.
We note that our calculations concerning the detection perspectives in gamma-rays are done 
assuming a $3$-year data acquisition period, with the region of interest being within the field-of-view
$100\%$ of the time. The same data acquisition period is used for antiprotons.


\subsubsection{Gamma-rays from intermediate galactic latitudes}
We have seen that the most common region of the sky that is examined in the literature as a source of $\gamma$-rays
is the galactic center, since it is the region where $N$-body simulations predict a maximization
of the dark matter density distribution and, hence, the corresponding gamma-ray flux.
However, the galactic center is quite poorly
understood as a region: there are large uncertainties in the background modelizations as well
as the density profile itsself. 

It has been proposed (see, for example, ref.\cite{Stoehr:2003hf}) that one could maximize the
signal/background ratio by actually excluding the region aroung the galactic center. Following
this reference, we perform our computations in a conoidal region extending from $20^\circ$ up to 
$35^\circ$ from the galactic center, excluding at the same time the regions within $10^\circ$ from the
galactic plane. It has actually been shown that within the framework of such an analysis, 
one can enhance the signal/background ratio by up to roughly an order of magnitude. The relevant
background for this region will be discussed in the next subsection.

In the meantime, we present in table \ref{JbarsLight} the values obtained for the $\bar{J}$ quantity
defined in eq.(\ref{Jbar}), for the three different halo profiles also discussed in the BMSSM analysis:
the Navarro, Frenck and White one, the Einasto profile and a NFW-like profile that has tried to take into account
the effects of baryons in the inner galactic regions.

\begin{table}
\begin{center}
\begin{tabular}{|c|ccccc|}
\hline
 & $a$ [kpc] & $\alpha$ & $\beta$ & $\gamma$ & $\bar{J}$\\
\hline
Einasto &  -   &   -   &       &   -    & $ 10.486$\\
NFW     & $20$ & $1.0$ & $3.0$ & $1.0$  & $8.638$\\
NFW$_c$ & $20$ & $0.8$ & $2.7$ & $1.45$ & $ 12.880$\\
\hline
\end{tabular}
\caption{{\footnotesize Einasto, NFW and NFW$_c$
density profiles with the corresponding parameters,
and values of $\bar{J}(\Delta\Omega)$ for the galactic
region under consideration.}}
\label{JbarsLight}
\end{center}
\end{table}
The $\bar{J}$ values obtained in the table demonstrate another virtue of searching
for dark matter at intermediate latitudes, namely the fact that the results become
quite robust with respect to the various dark matter density distribution
modelizations. We saw in all previous analyses that in the galactic center case, there can be differences of
orders of magnitude in this factor, whereas in this case the differenes are of
$O(1)$. In the following, we shall be presenting our results for an Einasto
profile, since it yields results somewhere in the middle among the other two
scenarios.

The Fermi collaboration has published its 1-year observation results outside the GC
\cite{Abdo:2010nz, Porter:2009sg, Abdo:2009mr}. In this paper, the collaboration presents its
observations for a period of $19$Msec and for various galactic latitudes. 
In the companion paper, the results for latitudes $20^\circ<b<60^\circ$ are
also presented, which lie actually in our region of interest. The data between $b = 10^\circ$ and
$20^\circ$ are included in the same paper, presenting an enhancement by a factor of roughly 
$1.5 - 2$  with respect to the higher latitude data. In this analysis, 
for the sake of simplicity, we shall
be focusing on the data from higher latitudes ($20^\circ<b<60^\circ$), integrating them over the whole
region of interest. This is  justified, since we have excluded 
from our analysis the region within $20^\circ$ from the galactic center, which should provide
one of the major contributions to this spectrum.

In the paper, the authors could fit the data quite well using a Diffuse Galactic
Emission model based on the GALPROP code. We find this model to be well reproduced, in our 
region of interest, by a simple power-law
\begin{equation}
 \Phi_{\mbox{\begin{tiny}bkg\end{tiny}}}^{\mbox{\begin{tiny}Th\end{tiny}}} = 2.757\cdot 10^{-6} E^{-2.49}
\end{equation}
in units of GeV$^{-1}$ sec$^{-1}$ cm$^{-2}$ sr$^{-1}$.

In the same analysis, the collaboration presents the detector effective area values 
that should be used in order to compare predictions with observations, as a function of
the gamma-ray energy. In the following, we shall be using these values rather than the usual
nominal effective area of $10000$ cm$^2$.
We consider a $3$ - year data acquisition period under the previous assumptions.

\subsubsection{Antiproton detection}
The assumptions concerning the astrophysical and experimental setup that we consider in this analysis
are exactly the same as in the BMSSM study presented previously. We take the data acquisision
period as $3$ years. We perform our calculations for the three propagation models MIN, MED
and MAX as defined previously. We shall only be showing our results on the MED model, since it
constitutes an intermediate scenarion, and comment upon the results on the other two 
propagation models.

\subsubsection{Results for indirect detection}
In order to characterize parameter space points as excluded or detectable, we calculate the
minimal boost that would be needed in the total self-annihilation cross-section in order to
satisfy conditions (\ref{exclusion}) or (\ref{detectabilityCriterion}) respectively. 
In other words, by maintaining the
mass and branching fractions of each parameter space point as in our model, we calculate the
minimal $<\sigma v>$ value that would be needed for the point to be excluded or detectable, and then
divide by it the actual corresponding cross-section predicted by the model. If this coefficient is 
smaller or equal to $1$, the corresponding point is excluded/detectable whereas in the opposite
case it is not.
\\ \\
As a first remark, we note that according to our findings no point of our parameter space is 
excluded. The cross-sections are too low. From now on, we shall therefore stick to predictions 
concerning the detection perspectives as described in the previous paragraphs.
\\ \\
In fig.\ref{a01100}, appart from the information mentioned previously, we also 
plot the contours where the boost required for a positive detection 
becomes equal to $1$ for the light neutralino scenario. We denote it by $D_\gamma$ and 
$D_{\mbox{\begin{tiny}MED\end{tiny}}}$ for the cases of gamma-rays 
and antiprotons, assuming an Einasto profile and the MED propagation model respectively. The contours for
gamma-rays are blue-dashed whereas for antiprotons violet-dotted. All parameter space points lying among the 
two lines which are quasi-symmetric around the rennonance are -in principle as we explained- detectable.
The same happens for the points lying on the left of the blue line for small $m_{1/2}$ values which is almost
parallel to the $m_A$ axis.
We note that in the case of gamma-rays, switching to another profile does not significantly alter the results.
In the case of antiprotons however, the results \textit{do} change. 
We have further calculated that for the MIN propagation model defined previously the whole 
parameter space evades detection, whereas for the MAX all viable points fall well within the detectable region.
\\ \\
Before explaining these results, we make the introductory remark that as can be seen for example in \cite{Baltz:2008wd}, the Fermi
satelite should in principle be able to exclude WIMPs with thermal cross-sections lying in our neutralino
mass range and for $b \bar{b}$ final states. Furthermore, these estimates were extracted having in mind
the Galactic Center as observation region. We already mentioned that it is considered that looking \textit{around}
this region can further improve the observation perspectives.
\\ \\
Concerning our results now, it is interesting that practically all of our points offer quite 
good detection perspectives. This is related to 
two facts: firstly, the present values of the annihilation cross-sections 
for the parameter space points passing the WMAP constraints
are quite high, namely of the same order as during decoupling (i.e. in the thermal region). This, in its turn, is
mainly due to the mechanism through which the correct relic density is actually obtained. 

We already saw that in
this scenario the mechanism that drives neutralino annihilation is resonnant $s$ - channel pseudoscalar higgs boson
exhange, apart from the small region at low $m_{1/2}$ and large $m_A$, where the dominant mechanism is CP-odd light
higgs exchange. In the case of annihilation through an $A$ propagator, the cross-section is practically insensitive to
velocity changes as pointed out for example in \cite{Jungman:1995df} and demonstrated in Appendix \ref{FeynmanGraphs}. 
This leads to the conclusion that the
self-annihilation cross-section stays quite large even at present times. It is really instructive to compare
this regime with the corresponding points where the relic density calculation is driven by annihilation into
$h$. In that case, $<\sigma v>$ tends to zero as the LSP velocity does so (i.e. at present times, which are relevant
for indirect detection experiments). 

This is indeed an interesting
effect, which renders the $h$-pole points practically invisible to indirect detection experiments. 
If one observes the indirect detection results for the BMSSM, one can deduce that 
detectability limits (although defined
differently) seem to systematically ``avoid'' the $h$-pole region. Furthermore, we should note that
the decay modes in our LHS are dominated by the $b \bar{b}$ final state. This is due first of all to kinematics but also
to the fact that annihilation into $A$ and then into down-type fermions 
is proportional to the quark mass, through the dependence of the 
relevant amplitude on the Yukawa couplings. We have seen that this is a final state
yielding relatively rich photon spectra if compared, for example, to the leptonic case. 
This is less the case for the antiproton yield, where the decays of light quarks have the tendency of
yielding more antiprotons than $b \bar{b}$ pairs.
Furthermore, there is also some $\tau^+ \tau^-$ component, which in the case
of gamma-rays gives some smaller contribution but in the case of antiprotons eliminates entirely some
fraction of the -potential- spectrum. This could be an explanation of the relatively better 
detection perspectives at Fermi than at AMS-02 - we remind however that we have calculated that if we instead
plotted the results for the MAX model the detectability regions are of the same order of magnitude.
\\ \\
Let us now proceed to our second scenario, i.e. fig.\ref{a01000}. Once again, 
the blue-dashed line depicts points where $D^\gamma = 1$ whereas the violet-dotted one represents
$D_{\mbox{\begin{tiny}MED\end{tiny}}} = 1$. Astrophysical assumptions are the same as in the previous case. Points lying 
above, below or on the left of the contours are detectable. If we plotted the gamma-ray results for the
other two profiles we examined, results would be practically unchanged. In the case of the two other
propagation models for antiprotons, the MAX model renders the entire parameter space visible whereas
in the MIN model AMS-02 will be blind to all of our points, with the points favouring positive detection
lying mostly above and on the left the WMAP-compliant region. We can see that in this scenario, the 
perspectives are also quite good. Once again, we should note that we are still lying 
in the $A$-pole region: the relic density calculation
is driven by the $s$-channel pseudoscalar exchange. Once again, $<\sigma v>$ lies roughly in the 
typical thermal region. But in this case, the lightest neutralino has a higher mass than previously.
This is the reason why we see that for relatively large values of $m_{1/2}$ and $m_A$ we have a certain
deterioration in the antiproton channel. Although less manifest, this is also the case in fig.\ref{a01100}.
And, if we observe the gamma-ray detectability lines carefully, it can also be seen that this line is
also characterized by the same tendency.

We should further note that in this parameter space region, there can be quite sizeable contributions
from final states including higgses and gauge bosons. Especially the latter, whereas they do not 
have an impact on the detection of gamma-rays (assuming same masses as in the $b \bar{b}$ case), 
they \textit{do} disfavour antiproton detection.

It is interesting to note that in both benchmarks, the Light Higgs scenario falls within the
detectable zone in both channels. This is due exactly to the combination of a relatively high
value for the self-annihilation cross-section at zero velocity and the fact that in this region both the
higgses as well as the lightest neutralino are very light.
\\ \\
In our two scenarios we examine two regimes, one with a quite light neutralino 
($50 \lesssim m_{\chi_1^0} \lesssim 70$ GeV) and one with a relatively heavier one
($100 \lesssim m_{\chi_1^0} \lesssim 130$ GeV), finding that a good part of our parameter
space should be visible at Fermi and AMS-02 (always according to our definitions). There is, 
however, one question that could be posed, namely what happens in the intermediate mass regime.
The answer could be given once more by considering that it is well-known that
increasing the WIMP mass tends to aggravate detection perspectives, if the same final states and
self-annihilation cross-section are assumed. Both the $Br_i$'s and $\left\langle \sigma v \right\rangle$
remain quite stable in value from lighter to higher masses in our model: the final state is mostly $b \bar{b}$
and the cross-section is of the typical thermal value, both during decoupling \textit{and} at present times.
We have thus no reason to expect that in the intermediate mass regime something spectacular should
happen altering the detection perspectives. Overall, this $A$-pole scenario that we have examined
can be considered as quite promising for indirect detection.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Direct detection in the NUHM model}
In fig.\ref{DirectLimits} we scatter the WMAP-compliant parameter
space points on the $(m_\chi, \sigma_{\chi-N}^{SI})$ (neutralino mass - neutralino-nucleon spin-independent
scattering cross-section) plane and compare them against the three strongest bounds available in the 
literature: The combined 2008 and 2009 CDMS-II results, the constraints from the XENON10 experiment as
well as the latest bounds from XENON100. We take the two former ones from ref.\cite{Kopp:2009qt} and the
latter from \cite{Aprile:2010um}. We further highlight the points falling into the light higgs scenario
defined throughout this paper with different colors.

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=10cm,height = 15cm,angle=-90]{./susy/directLimitsNOlogm.eps}\\
\end{center}
\caption{{\footnotesize
$(m_\chi, \sigma_{\chi-N}^{SI})$ combinations occuring in the parameter space region
under examination, along with some of the relevant exclusion limits from some direct detection
experiments. The points lying above the lines are in principle excluded according to the published
limits. Yellow points correspond to a trilinear coupling value of $A_0 = -1000$ whereas pink ones to
$A_0 = -1100$. We highlight by light blue and dark blue the points lying in the
Light Higgs Boson regime respectively for the two scenarios. 
Limits from experiments weaker than the ones presented here are omitted.
}}
\label{DirectLimits}
\end{figure}

We see that many of our points fall largely within the region that is supposed to be excluded
from the existing data. Whereas the $A_0 = 1100$ scenario (pink points) is more or less satisfying the constraints,
the scenario with $A_0 = 1000$ (yellow points) is in most cases largely above the limits, exceeding even
by more than an order of magnitude the CDMS-II and XENON100 allowed cross-sections. In both cases, 
the points satisfying the light higgs criteria fall within the excluded zones.

However, in chapter \ref{Chapter2} it was mentioned that there can be significant uncertainties
that complicate the assertion on whether a particular model is excluded or not. More specifically:
\begin{itemize}
 \item Uncertainties can arise in the calculation of the neutralino-nucleon elastic scattering cross-section,
which can be due to a number of factors. As an example, as described in
detail in \cite{Ellis:2008hf}, significant uncertainties can arise in the passage from the parton-level cross-section
to the hadronic level one. 
 \item Some uncertainty might be present in the passage from the hadronic to the nuclear level. Indeed, 
at the end of the day the primarily constrained quantity is the WIMP-\textit{nucleus} elastic scattering cross-section
and not the WIMP-\textit{nucleon} one. It would not thus be impossible to think that the nuclear form factors
could be a source of some error.
 \item The local dark matter density is by no means a perfectly well known quantity and is in fact a normalization
factor in the overall procedure of computing the WIMP-nucleus scattering rate.
 \item Little is known on the true velocity distribution of WIMPs in the detector rest frame as well as on the
escape velocity at which the integral over the velocity distribution should be truncated.
\end{itemize}
The first point concerns our calculation of the spin-independent
neutralino-nucleon elastic scattering cross-section. In other words, and refering to fig.\ref{DirectLimits}, we 
expect that a certain variation in the position of parameter space points on the $(m_\chi, \sigma_{\chi-N}^{SI})$ plane
should be allowed. 
The other remarks apply to the experimental limits published
from the various collaborations, i.e. they can amount to a change in the position of the exclusion lines. 

Overall, and despite the apparent exclusion of a large portion of our parameter space, there is still
quite some margin for changing the relation among the predicted $(m_\chi, \sigma_{\chi-N}^{SI})$ as derived
from the model and the exclusion limits as presented by the corresponding collaborations. We feel it is
reasonable to say that we cannot assess that easily whether the parameter space points lying above the exclusion
lines in fig.\ref{DirectLimits} are act actually excluded or not.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%










==> susy/MySUSY.tex <==
\section{Beyond the MSSM}

\subsection{The framework}
One of the first thoughts that might come in mind in an effort to satisfy the LEP2
bounds could be to further extend the particle content of the MSSM. New contributions
to the lightest Higgs mass could in principle raise the tree-level (or even the loop-level)
prediction and conciliate it with the experimental constraints. Numerous such examples
are known in the literature. An important issue is, however, that nothing is
known about what could be the physics beyond the MSSM (IF the MSSM has something to do
with physical reality).

During the last few years, a series of papers 
\cite{Strumia:1999jm, Brignole:2003cm, Casas:2003jx, Pospelov:2005ks, Pospelov:2006jm, Dine:2007xi} 
have followed a somewhat alternative
approach: Instead of examining all possible extensions of the MSSM, one could just assume that
new physics enters the game at some scale $M$, imposing a cutoff to the theory. Below this 
cutoff, the new degrees of freedon can in principle be integrated out of the theory resulting
in an effective lagrangian near the EW scale. The new operators can then be organized according
to their suppression by the cutoff scale in the superpotential. 
Dimension - $5$ operators will be suppressed as $1/M$, 
dimension - $6$ as $1/M^2$ and so on.

At first sight, the number of potential operators that one could include in
order to write down the most general dimension five superpotential is huge, not to speak of
higher - dimensional operators. However, it turns out that employing superfield techniques and
identities, the total number of these operators can be significantly reduced by redefining 
a certain number of them. In fact, the most general dimension - $5$ \cite{Antoniadis:2008es} 
and dimension - $6$ \cite{Antoniadis:2009rn} MSSM
superpotentials were recently written down. Several new parameters and contributions should
be taken into account, but apparently much less than one would have initially expected.

In the light of the previous discussion on the little hierarchy problem, one could start with 
a little less ambition and strictly try to address the higgs mass issue, for example by only
including dimension - $5$ operators only involving Higgs fields. This was done quite recently 
by Dine, Seiberg and Thomas in ref.\cite{Dine:2007xi}. Baryon and lepton number violating operators
are ignored, as is done for operators that could be added in the squark sector.

The authors found a remarkable result, namely that there are only two independent operators 
falling under the previous considerations that can be added to the MSSM superpotential.
The first of these operators is supersymmetric:
\begin{equation}
 W_5^{\mbox{\begin{tiny}SUSY\end{tiny}}} = \frac{\lambda_1}{M} (H_u H_d)^2
\label{BMSSMsusypres}
\end{equation}
Another contribution comes from supersymmetry breaking terms. This operator can be written as
\begin{equation}
 W_5^{\cancel{\mbox{\begin{tiny}SUSY\end{tiny}}}} = \frac{\lambda_2}{M} {\cal{Z}} (H_u H_d)^2
\label{BMSSMsusybreak}
\end{equation}
where ${\cal{Z}}$ is a supersymmetry breaking
spurion field, ${\cal{Z}} = m_{\mbox{\begin{tiny} SUSY\end{tiny}}} \theta^2$. Here, 
$m_{\mbox{\begin{tiny} SUSY\end{tiny}}}$ is the supersymmetry breaking scale.
\\ \\
The total superpotential for this model (dubbed Beyond the MSSM, BMSSM) is, of course, the
sum of the three contributions
\begin{equation}
 W_{\mbox{\begin{tiny}BMSSM\end{tiny}}} = 
W_{\mbox{\begin{tiny}MSSM\end{tiny}}} + 
W_5^{\mbox{\begin{tiny}SUSY\end{tiny}}} +
W_5^{\cancel{\mbox{\begin{tiny}SUSY\end{tiny}}}}
\label{BMSSMsuperpotential}
\end{equation}
Differentiating the superpotential with respect to the theory's scalar fields and then
squaring, we can get the Higgs scalar potential. This shall include both $1/M$
and $1/M^2$ - suppressed terms, of which according to our discussion we only keep the
former, i.e. the crossed terms between the MSSM contribution and the new pieces.
The supersymmetric and supersymmetry breaking parts give us the following contributions
respectively
\begin{eqnarray}
 \delta V_1 & = & 2 \epsilon_1 (H_u H_d) (H_u^\dag H_u + H_d^\dag H_d) + h.c.\\
 \delta V_2 & = & \epsilon_2 (H_u H_d)^2 + h.c.
\label{BMSSMscalarcontr}
\end{eqnarray}
where we have defined the two new parameters that the model introduces
\begin{eqnarray}
 \epsilon_1 & \equiv & \frac{\mu^* \lambda_1}{M}\\
 \epsilon_2 & \equiv &  - \frac{m_{\mbox{\begin{tiny} SUSY\end{tiny}}} \lambda_2}{M}
\label{BMSSMparameters}
\end{eqnarray}
Finally, the new operators introduce a new Higgs-Higgs-higgsino-higgsino interaction 
lagrangian
\begin{equation}
 \delta{\cal{L}} = - \frac{\epsilon_1}{\mu^*}
\left[
2 (H_u H_d) (\tilde{H}_u \tilde{H}_d) + 
2 (\tilde{H}_u H_d) (H_u \tilde{H}_d) + 
  (H_u  \tilde{H}_d) (H_u \tilde{H}_d) + 
  (\tilde{H}_u H_d) (\tilde{H}_u H_d)
\right] + h.c.
\label{BMSSMinteractions}
\end{equation}
This contribution modifies the higgsino annihilation process, which
can be relevant for dark matter phenomenology provided the neutralino has a significant higgsino
component. 

At the same time, all of the above contributions modify the relation among the higgs
mass and the stop sector, as well as the neutralino and chargino masses. Concerning the
lightest higgs mass, the Non - Renormalizable (NR) corrections to the higgs mass can become sizeable, allowing
to satisfy the LEP2 limits even at tree-level for moderate stop mass values and without
substantial left-right stop mixing. The modifications in the lightest higgs mass, the neutralino
mass matrix, as well as in some useful couplings can be found along with some other useful
formulae in Appendix \ref{NeutralinoCouplings}.
\\ \\
Several aspects of the model have been studied in the literature
\cite{Blum:2008ym, Cheung:2009qk, Cassel:2009ps, Carena:2009gx, Bernal:2009hd}.
Since the model is much more extended and complex than the singlet scalar one, we shall
not describe in as much detail its various phenomenological consequences and constraints.
For the sake of brevity, we shall only focus on the dark matter - related phenomenology.
The first step is to describe the relic density constraints coming from the WMAP measurements.
Then, we shall present some work effectuated in \cite{Bernal:2009jc} concerning the dark matter 
detection prospects for the model.

\subsection{Relic Density}
The impact of the NR operators on the relic density calculation has been examined in detail in
references \cite{Berg:2009mq} and \cite{Bernal:2009hd}. In both of these papers, the authors
scan over the BMSSM parameter space (the conventions used in the two papers are different), 
finding WMAP - compliant regions that are absent in the MSSM case, either due to the ellimination
of a number of them by ``external'' constraints, or because the MSSM just cannot produce the 
relevant phenomenology.

We shall be examining the dark matter phenomenology in the two benchmark scenarios
discussed in \cite{Bernal:2009hd}: the first one tries to compare the BMSSM phenomenology
with the low-energy phenomenology of a typical CMSSM model, whereas the second one 
begins with the definition of a low-energy model which in the BMSSM framework can lead
to light stops and heavy sleptons.

\subsubsection{Correlated stop - slepton masses}
\label{CorrSSmasses}
The first scenario of \cite{Bernal:2009hd}  begins with the typical set of the five free parameters present in
CMSSM - like models
\begin{equation}
 \tan\beta, \ m_{1/2}, \ m_0, \ A_0, \ \mbox{sign}(\mu)
\end{equation}
In such a framework, the low energy parameters can be approximately given by
\begin{eqnarray}
 m^2_{\tilde q}&\approx&m_0^2+6\,m_{1/2}^2,\nonumber\\
m^2_{\tilde\ell_L}&\approx&m_0^2+0.5\,m_{1/2}^2,\nonumber\\
m^2_{\tilde\ell_R}&\approx&m_0^2+0.15\,m_{1/2}^2,\nonumber\\
M_1&\approx&0.4\,m_{1/2},\nonumber\\
M_2&\approx&0.8\,m_{1/2},\nonumber\\
M_3&\approx&3\,m_{1/2}.
\end{eqnarray}
Three out of the five parameters of the CMSSM model are fixed, choosing
specifically $\tan\beta = 3$ or $10$, $A_0 = 0$, $\mbox{sign}(\mu) > 0$ and then 
the remaining $(m_0, m_{1/2})$ parameter space is scanned and the relic density as
well as a number of EW observables are computed.

The resulting low-energy model is next enriched with the addition of the NR operator
contributions and the observables are recalculated. We should stress at this point
that the new framework should \textit{by no means} be conceived as a generalized 
CMSSM model, since it is impossible to take into account the BMSSM physics effects
on the running of physical quantities from the GUT scale down to the electroweak scale:
the two models are compared \textit{only} with respect to their low-energy phenomenology.

In order to present the relic-density related phenomenology, we borrow fig.\ref{fig:BMSSMrelic}
from ref.\cite{Bernal:2009hd}. In this figure, the left-hand side plot corresponds to the
CMSSM benchmark with the BMSSM contributions set to zero.
The WMAP - compliant regions are delimited by red solid lines (in practice the regions seem
as lines in the plot). Furthermore, a series of constraints are also depicted in the figure:
the regions above and on the left of the yellow dashed lines correspond to a non-neutralino
LSP (in this case it is the stau), the regions below the blue dotted line are excluded by the null
chargino searches at LEP whereas the black dotted-dashed lines are light higgs mass isocontours
as seen in the figure. We note that the entire parameter space depicted in the figure is 
in any case excluded due to the lightest higgs mass constraint.

\begin{figure}[htb]
\vspace{2cm}
\begin{center}
\hspace{-4cm}
\includegraphics[width = 5cm]{./susy/mS3-0.eps}
\hspace{3cm}
\includegraphics[width = 5cm]{./susy/mS3-1-5.eps}
\caption{{\footnotesize
Regions in the $(m_0, m_{1/2})$ plane where the WMAP constraints are satisfied (red solid regions)
in the case of a plain CMSSM (left panel) and a BMSSM (right panel) model. The regions below the blue
dotted lines are excluded by null searches for charginos at LEP. The regions to the left and above
the yellow dashed lines are excluded due to stau LSP. Finally, the black dotted-dashed lines are
light higgs mass contours in GeV.}}
\label{fig:BMSSMrelic}
\end{center}
\end{figure}

Once the low-energy spectrum and observables are computed, the next step is to turn on the
BMSSM contributions. In the original paper this is done in two steps: first, only the 
$\epsilon_1$ parameter is turned on choosing $\epsilon_1 = -0.1$ and $\epsilon_2 = 0$.
We point out that in our notations, a negative $\epsilon_1$ value yields a positive 
contribution to the lightest higgs mass, as can be verified in Appendix \ref{NeutralinoCouplings}.
Everything is recalculated with this configuration. Then, both parameters are given
non-zero values, namely $\epsilon_1 = -0.1$ and $\epsilon_2 = 0.05$ and the process is
repeated. For the time being, we ommit the intermediate step with $\epsilon_2 = 0$
and just give the results with both parameters turned on (right panel of fig.\ref{fig:BMSSMrelic}).
Later, when discussing the BMSSM dark matter detection issue, we shall present all three
configurations. A first remark that could be already made for the BMSSM variant is that  the
LEP2 higgs mass bound is immediately satisfied for the entire parameter space thanks
to the contributions from the new operators.

Let us now start the description of the relic density results with the left panel, 
i.e. the plain mSUGRA model (forgetting
for the moment that it is in any case excluded). As a general rule, we could
say that the model tends to yield too small neutralino self-annihilation cross-sections and thus
overproduce dark matter. At low $m_{1/2}$ values and almost parallel to the $m_0$ axis, we notice
two stripes where the WMAP bounds are satisfied. These are around the region where the neutralino
mass is close to half the mass of the lightest higgs boson or the $Z$ boson, 
$m_{\chi_1^0} \sim m_{h, Z}/2$. In this regime, the neutralino self-annihilation cross-section
gets enhanced because the light higgs propagator in the $s$ - channel starts being nearly on-shell.
The second region of interest is the one almost parallel to the stau LSP constraint line, at low
$m_0$ values. In this region, the correct relic density is obtained not because of some enhancement
in the neutralino self-annihilation cross-section, but due to efficient $\chi_1^0$ - $\tilde{\tau}$ 
coannihilation. Finally, for small $(m_0, m_{1/2})$ values, we have the bulk region, where 
the relic density calculation is driven by crossed sfermion exchange.

The most striking feature brought about by the introduction of the NR operators (right-hand side plot) 
is the appearence
of a new, distinct zone where the relic density constraint is satisfied. This is the region again
almost parallel to the $m_0$ axis and above the chargino LEP exclusion limits. In fact, this region 
is not exactly new: the introduction of the dimension - $5$ operators has the effect (and the aim)
to raise the higgs mass. Hence, whereas in the CMSSM case the $Z$ and $h$ pole regions are 
practically degenerate, the new contributions uplift the higgs mass causing for the seperation
of the two resonnant regions. And whereas the $Z$ pole region remains excluded by the LEP
chargino search limits, the $h$ pole region is now perfectly viable.


\subsubsection{Light stops, heavy sleptons}
\label{LSHS}
The second scenario introduced in \cite{Bernal:2009hd} makes no reference whatsoever to GUT-scale
conditions (even if in the previous case we are not interested in them either). The authors start
with a set of low-energy parameters, namely 
\begin{equation}
 M_2,\ \mu,\ \tan\beta,\ X_t,\ m_U,\ m_Q, \ m_{\tilde f},\ m_A,
\end{equation}
which correspond respectively to the Wino mass, the higgsino mass parameter, the usual ratio 
of the Higgs vacuum expectation values, the trilinear coupling - dependent parameter $X_t=A_t- \mu \cot \beta$, 
the right stop mass parameter, a common mass parameter for the third generation 
left squarks, a common mass for the sleptons, the first two generation squarks and the 
right sbottom and, finally, the pseudoscalar mass. Six out these eight parameters are fixed as
$\tan\beta=3$ or $10$, $X_t=0$, $m_U=210$ GeV, $m_Q=400$ GeV,
$m_{\tilde f}=m_A=500$ GeV and a scan is performed in the $(M_2, \mu)$ parameter space.
Then, the $\epsilon_1$ and $\epsilon_2$ parameters are turned on as in the previous scenario
(choosing $\epsilon_1=-0.1$ and then also $\epsilon_2=+0.05$) and the scan is repeated.
\\ \\
This scenario is chosen in order to yield light stops
\begin{equation}
 m_{\tilde t_1}\lesssim 150\ {\rm GeV},\ \ \ \ 370\
{\rm GeV}\lesssim m_{\tilde t_2}\lesssim 400\ {\rm GeV}
\end{equation}
which, as argued in the paper, is a favourable scenario for electroweak baryogenesis.

\begin{figure}[htb]
\vspace{2cm}
\begin{center}
\hspace{-4cm}
\includegraphics[width = 5cm]{./susy/tb3-0.eps}
\hspace{3cm}
\includegraphics[width = 5cm]{./susy/tb3-1-05.eps}
\caption{{\footnotesize
Regions in the $(M_2, \mu)$ plane where the WMAP constraints are satisfied (red solid regions)
in the case of a plain MSSM (left panel) and a BMSSM (right panel) model. The regions below and on the 
left of the blue
dotted lines are excluded by null searches for charginos at LEP. The regions to the right and above
the yellow dashed lines are excluded due to stop LSP. The violet curve in the right panel
depicts constraints coming from vacuum stability.
}}
\label{fig:BMSSMrelicLSHS}
\end{center}
\end{figure}
We once again borrow fig.\ref{fig:BMSSMrelicLSHS} from \cite{Bernal:2009hd} in order to 
describe the relic density phenomenology.
We start with the plain MSSM model (left panel). The first regions where the WMAP constraints are satisfied
are the two red regions at roughly $M_2 \approx 100$ GeV and almost parallel to the
$\mu$ axis. These correspond to neutralino annihilation taking place near the $h$ and $Z$ poles
as before. Around these regions the relic density is too high, whereas between them it is
too low. The next region is the one quasi-parallel to the neutralino LSP constraint, where 
the driving mechanism enhancing the neutralino annihilation process is coannihilation with the 
NLSP, which in this case is the lightest stop. Finally, there is one last region around $M_2 \sim 200$ Gev
and $\mu \sim 250 - 300$ GeV, where the neutralino starts acquiring a significant higgsino fraction, 
augmenting its couplings to the $Z$ boson and amounting mostly to gauge and higgs boson final states.
Interestingly, for larger $M_2$ values the self-annihilation cross-section becomes too large, 
and the lower WMAP limit is violated.

Introducing the dimension - $5$ operators has, once again, mainly the effect of seperating the $h$
and $Z$ pole regions, due to the rise in the lightest higgs mass. Once again, the $h$ pole region
evades the LEP chargino search limits. Finally, we remark the appearence of a violet line at large
$\mu$ values. This corresponds to a further constraint, which is the requirement for
vacuum stability. Indeed, in the presence of the NR operators the scalar Higgs potential can
get destabilized, with a second remote vacuum forming, rendering the EW breaking vacuum of the theory
metastable.

Having discussed the two scenarios and their relic density - related phenomenology, we can now 
proceed to examine the detection prospects for the model in various channels.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Dark matter detection in the BMSSM}
In ref.\cite{Bernal:2009jc} we examined the detection perspectives for the two BMSSM models
presented previously. Finding first the WMAP-compatible regions (to be depicted in red
in the plots that follow), 
we estimated whether the parameter space points for the two scenarios
can be probed using four different detection techiques: direct detection in a XENON - like
experiment, gamma-ray detection at the Fermi satelite mission as well as positron and
antiproton detection coming from DM annihilations in the AMS-02 experiment.

The method we followed was to first compute the detection rates with $\epsilon_1 = \epsilon_2 = 0$, 
i.e. in the plain MSSM case. This shall correspond to the first row in all plots that follow
for this study. Then, we further examine two BMSSM variants for each scenario, 
turning on the values $(\epsilon_1 = -0.1, \epsilon_2 = 0)$ (second-row plots) and 
$(\epsilon_1 = -0.1, \epsilon_2 = 0.05)$ (third-row plots) in each one of them. Our computations were done assuming
two distinct values for $\tan\beta$, namely $3$ and $10$. The first case shall correspond to the left-hand
side plots, whereas the second one to the right-hand side ones.

Before presenting our results, it is useful to define what we shall be 
meaning in this treatment when we characterize
a parameter space point as being ``detectable''.
We employ a method based on the $\chi^2$ quantity.
Consider whichever mode of detection: direct or indirect in any of the three channels
($\gamma$-rays, $e^+, \bar{p}$) we shall be considering. In all four modes, what 
is finally measured is a number of events per energy bin.
Let us call $N^{sig}_i$ the number of signal (dark matter - induced) events in
the $i$-th bin, the nature of which depends on the specific experiment, 
$N^{bkg}_i$ the corresponding
background events in the same bin, and $N^{tot}_i$ the sum of the two.
The variance $\chi^2_i$ in every bin is defined as:
\begin{equation}
\chi^2_i =
\frac{(N_i^{tot}-N_i^{bkg})^2}{N_i^{tot}} \ .
\end{equation}
Then, the condition that we impose to characterize a point as detectable, is that at least 
in one energy bin 
$\chi^2_i\gtrsim 5.8$. In Gaussian error terms, this corresponds to a $95\%$ CL.

We shall now present the work effectuated for each of the four detection modes, introducing
our experimental and theoretical assumptions and simplifications, then describing the
results for each of our two models.


\subsection{Direct detection}
The first part of the work consists of calculating the regions of our parameter space that can
be probed in a XENON-like experiment for our twelve models (2 scenarios each with 6 sub-variants
as described before).
To this goal, we consider $7$ recoil energy bins 
between $4$ and $30$ keV. The background in this analysis is set
to zero. Furthermore, we assume three exposure values (time $\times$ detector mass) which we take
as $\epsilon = 30, 300$ and $3000$ kg$\cdot$year. These exposure values could correspond e.g. 
to a detector with $1$ ton of xenon and $11$ days, $4$ months or $3$ years of data acquisition, respectively.

Concerning astrophysics, in this analysis we take the standard halo model with neutralinos
following a Maxwell-Boltzmann velocity distribution in the galactic rest frame and neglecting the
motion of the earth around the sun, whereas the local DM density is set to $0.385$ GeV cm$^{-3}$. 
The sun's velocity around the GC is set to $220$ km sec$^{-1}$.

\subsubsection{Correlated stop-slepton masses}
Figure \ref{dir1} shows the sensitivity lines (black lines) for 
exposures $\varepsilon=30$, $300$ and $3000$ kg$\cdot$year, 
on the $[m_0,\,m_{1/2}]$ parameter space, for all other parameters as defined in paragraph \ref{CorrSSmasses}.
We repeat for the sake of convenience that
the first-row plots correspond to plain CMSSM scenarios whereas the second and third to the
`mSUGRA-like' benchmark, with the $\epsilon_1$ and $(\epsilon_1, \epsilon_2)$ parameters turned on 
respectively.
The plots on the left correspond to a choice $\tan\beta = 3$ whereas the right-hand side ones
to $\tan\beta = 10$.
These curves reflect the XENON sensitivity and represent its ability to test and 
exclude different regions of the mSUGRA and BMSSM relevant model at $95\%$ CL: 
all points lying below the black lines are detectable.
When some line is absent, this means that the whole parameter space can be 
probed for the corresponding exposure.

Some further information is included in the plot (as well as the ones to follow):
The red regions depict the parameter space points yielding relic densities compatible
with the WMAP limits.
The regions in orange (light gray) or blue (dark gray) are excluded
due to the fact that the LSP is the stau or because of the null searches for charginos
at LEP.
For large $\tan\beta$, an important fraction of the $[m_0,\,m_{1/2}]$ plane,
corresponding to the region above the violet line, generates an unstable vacuum
and is then excluded.
An interesting remark is that the introduction of $\epsilon_2$ alleviates the vacuum 
stability constraint \cite{Blum:2009na}, and slightly increases the Higgs mass.
\begin{figure}[tbp!]
\begin{center}
\vspace{-0.2cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dir3-0.eps}\hspace{0.2cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dir10-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dir3-1-0.eps}\hspace{0.2cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dir10-1-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dir3-1-5.eps}\hspace{0.2cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dir10-1-5.eps}
\end{center}
%\vspace{-0.9cm}
\caption{{\footnotesize
Regions in the $[m_0,\,m_{1/2}]$ plane that can be detected by XENON using exposures
$\varepsilon=30$, $300$ and $3000$ kg$\cdot$year, for our mSUGRA-like scenario. 
The black lines depict the detectability regions: the area below the lines can be probed.
Whenever a line is absent, this means that the whole parameter space can be tested
by the experiment. The blue and orange regions depict the areas that are excluded by
direct LEP chargino searches and the requirement for a 
neutralino LSP respectively. The area above the violet line is excluded by the
metastable vacuum constraint.}}
\label{dir1}
\end{figure}


As a general rule, we can see from all plots that 
the detection prospects are maximised for low values of the $m_0$
and $m_{1/2}$ parameters. For higher $m_0$ values, the masses of the
squarks in the internal propagators increase, causing the scattering cross-section to decrease.
In the same way, the increase of $m_{1/2}$ augments the WIMP mass and
leads to a deterioration of the detection perspectives.
On the other hand, the region of low $m_{1/2}$ is also preferred because in that case the
lightest neutralino is a mixed bino-higgsino state, favouring the $\chi_1^0-\chi_1^0-h$
and $\chi_1^0-\chi_1^0-H$ couplings, and thus the scattering cross-section. Let us recall
that a pure higgsino or a pure gaugino state does not couple to the Higgs bosons, as can be seen
in Appendix \ref{NeutralinoCouplings}.

On the other hand, by comparing the left- and right-hand figures, we can see that
the detection prospects are also maximised for low values of $\tan\beta$.
For large values, besides the increase of the lightest Higgs boson mass, the coupling
of the latter to a $\chi_1^0$ pair decreases significantly because it is proportional 
to $\sin 2\beta$, for $|\mu|\gg M_1$.

The introduction of the NR operators gives rise to an important deterioration of the detection prospects.
The main effect enters via the important increase in the lightest CP-even Higgs mass.
This behaviour is attenuated for larger values of $\tan\beta$, since 
the corrections to the Higgs masses are suppressed by $1/\tan\beta$ (see e.g. reference \cite{Dine:2007xi}).
On the other hand, the neutralino couplings are not really influenced by the NR operators
in this regime, since $\chi_1^0$ is mostly bino-like. So, the impact
on its couplings with Higgs bosons is marginal. 

It is important to note at this point that the deterioration in the detection perspectives, while
existing, is nevertheless relative: we must not forget that the plain MSSM scenarios presented
here are already excluded because of the light Higgs mass.

Concerning the plots in figure \ref{dir1}, an overall remark that can be made is that, 
even for low exposures, a sizable amount of the parameter space can be probed.
The XENON experiment will be particularly sensible to low values of $m_{1/2}$.
However, larger exposures could be able to explore almost the whole parameter space taken
into account.


\subsubsection{Light stops, heavy sleptons}
Figure \ref{dir2} shows the exclusion lines for XENON with exposures
$\varepsilon=30$, $300$ and $3000$ kg$\cdot$year,
on the $[M_1,\,\mu]$ parameter space for our LSHS scenario, 
with the other parameters as defined in section \ref{LSHS} for
$\tan\beta=3$ (left panel) and $10$ (right panel).
\begin{figure}[tbp!]
\begin{center}
\vspace{-0.2cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dirB3-0.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dirB10-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dirB3-1-0.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dirB10-1-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dirB3-1-5.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/dirB10-1-5.eps}\\
\end{center}
%\vspace{-0.9cm}
\caption{{\footnotesize
Regions in the $[M_1,\,\mu]$ plane that can be detected by
XENON for the scenario with light stops and heavy sleptons. 
The black lines depict the detectability regions for the corresponding XENON
detector with exposures
$\varepsilon=30$, $300$ and $3000$ kg$\cdot$year: the area below the lines can be probed.
Whenever a line is absent, this means that the whole parameter space can be tested
by the experiment. The blue and orange regions depict the areas that are excluded by
direct LEP chargino searches and the requirement for a 
neutralino LSP respectively. The areas above the violet lines are excluded by the
metastable vacuum constraints.
}}
\label{dir2}
\end{figure}
Here again, the experiment will be sensitive to the regions below the black contours.
It can be seen that in general, the detection prospects are maximised for low values of the $M_1$
and/or the $\mu$ parameters. These regions correspond to a light $\chi_1^0$.
Although this might not be obvious in the figure, we have further seen that 
the scattering cross-section is enhanced near the region
$M_1\sim\mu$. In this case, the lightest neutralino is a mixed bino-higgsino state,
favouring the $\chi_1^0-\chi_1^0-h$ and $\chi_1^0-\chi_1^0-H$ couplings.
Again, the detection prospects are also improved for low values of $\tan\beta$.
This is due to the fact that for $|\mu|\gg M_1$
the coupling between the LSP and the Higgs bosons is suppressed by
a factor $\sin 2\beta$.
We further checked that 
the first line of the figure (corresponding to the case without
the NR operators), besides being excluded by the Higgs mass, is partially ruled out
by the recent XENON10 \cite{Angle:2007uj} and CDMS \cite{Ahmed:2009zw} searches.

When introducing the dimension $5$ operators the detection prospects deteriorate, in a
similar way as in the last subsection. The main effect is again the rise of the lightest Higgs mass.
Furthermore, the $\chi_1^0-\chi_1^0-h$ coupling is suppressed.
The latter effect is very accentuated in the region where the LSP is higgsino-like.
It is interesting however to notice that, for the case of large $\tan\beta$,
almost the whole area that falls outside the reach of XENON for $\varepsilon=30$ kg$\cdot$year
is already excluded by the vacuum stability constraint 
(i.e. the region above the violet line).
It should be noted that the BMSSM scenarios evade the aforementioned constraints from XENON10
and CDMS.

This scenario seems to offer exceptionally good detection perspectives.
Even with middle exposures, XENON will be able to detect dark matter in the whole viable region
for all three benchmarks and in the two models. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Gamma - rays from the Galactic Center}
Next, we examine the capacity of the Fermi mission to detect gamma-rays from neutralino 
annihilations coming from the galactic center region. We calculate the corresponding fluxes
and extract detactability limits considering gamma-rays within a cone of 
$\Delta\Omega \approx 3\cdot 10^{-5}$ around the galactic center. Our results are computed for
three halo profile cases already discussed in the first chapter: the Navarro, Frenk and White one, 
the Einasto profile as well as 
a NFW - like profile including adiabatic compression effects. The relevant values for the 
$\bar{J}$ quantity are shown in table \ref{tabProfilesBMSSM}.

\begin{table}
\begin{center}
\begin{tabular}{|c|ccccc|}
\hline
 & $a$ [kpc] & $\alpha$ & $\beta$ & $\gamma$ & $\bar{J}(3\cdot10^{-5}$ sr$)$\\
\hline
Einasto &  -   &   -   &       &   -    & $6.07\cdot10^3$\\
NFW     & $20$ & $1.0$ & $3.0$ & $1.0$  & $8.29\cdot10^3$\\
NFW$_c$ & $20$ & $0.8$ & $2.7$ & $1.45$ & $5.73\cdot10^6$\\
\hline
\end{tabular}
\caption{{\footnotesize Einasto, NFW and NFW$_c$
density profiles with the corresponding parameters,
and values of $\bar{J}(\Delta\Omega)$.
The latter has been computed by means of a VEGAS Monte-Carlo integration
algorithm, imposing a constant density for $r\le 10^{-7}$kpc so as to 
avoid divergences appearing in the NFW-like profiles.}}
\label{tabProfilesBMSSM}
\end{center}
\end{table}

The energy range we examine is $[1, 300]$ GeV which we divide into $20$ logarithmically evenly 
spaced energy bins and calculate the chisquare quantities as previously. The assumed
data acquisition period is $5$ years.

Concerning the background, we take into account two sources already described in the second chapter:
The bright source nearly coincident with the Galactic Center as detected by the HESS mission, as
well as the HESS measurements of the diffuse gamma-rays in the area surrounding the GC.

\subsubsection{Correlated stop-slepton masses}

In figure \ref{gam1} we present our results concerning the detection perspectives at
the Fermi mission for the three halo profiles.
Fermi will be sensitive to the regions below the contours and, for 
$\tan\beta=3$, to the area inside the blob.

\begin{figure}[tbp!]
\begin{center}
\vspace{-0.2cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gam3-0.eps}\hspace{0.2cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gam10-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gam3-1-0.eps}\hspace{0.2cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gam10-1-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gam3-1-5.eps}\hspace{0.2cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gam10-1-5.eps}
\end{center}
% \vspace{-0.4cm}
\caption{\footnotesize{
Regions in the $[m_0,\,m_{1/2}]$ plane that can be detected by the
Fermi satellite mission for our mSUGRA-like scenario. 
The black lines depict the detectability regions for the corresponding halo profile assumptions 
and $5$ years of data acquisition: the area below and on the left of the lines can be probed.
The same applies to the top-resonance blob at $m_{1/2}\sim 450$ GeV appearing on the left-hand side
plots. For NFW and Einasto profiles, the model could not be tested.}}
\label{gam1}
\end{figure}

It can be seen that the detection prospects are maximised for low values of the $m_0$
and $m_{1/2}$ parameters. This is due to the fact that for higher $m_0$ values, the masses of the
squarks increase, causing the annihilation cross-section to decrease.
However, the growth of $m_{1/2}$ gives rise to the opening of some relevant production channels,
after passing some thresholds, increasing significantly $\langle\sigma v\rangle$.
These thresholds appear as features, especially in the left-hand side
plots, where the detectability lines follow a less smooth behaviour.

The first one corresponds to a light neutralino, with mass $m_\chi\sim m_Z/2$
($m_{1/2}\sim 130$ GeV). In that case the annihilation is done via the $s$-channel exchange
of a real $Z$ boson, decaying in hadrons ($\sim 70\%$), neutrinos ($\sim 20\%$) and charged
leptons ($\sim 10\%$). We can see that in this region, although it is excluded by the LEP constraints, 
the detection prospects are good.

The second threshold appears for $m_\chi\sim m_W$ ($m_{1/2}\sim 220$ GeV). The annihilation cross-section
is enhanced by the opening of the production channel of two real $W^\pm$ bosons in the final state.
This process takes place solely through chargino exchange, since both $Z$ and Higgs bosons
exchange are suppressed by taking the limit $v\to 0$. 
In fact, this feature is even more interesting:
right below the opening of the gauge boson final states, the detectability lines seem to ``avoid'' the
$h$-pole region, since the process $\chi_1^0 \chi_1^0 \rightarrow h \rightarrow f \bar{f}$ that
dominated at freeze-out and augmented the self-annihilation cross-section is an inefficient 
mechanism at present times, as discussed in Appendix \ref{FeynmanGraphs}. As the neutralino mass
increases a little, the chargino exchange process starts entering the game as the gauge boson
final state becomes accessible. And, contrary to annihilation into a $h$ propagator, the cross-section
for this process does not decrase so dramatically as $v\to 0$.

The last threshold corresponds to the opening of the channel $\chi_1^0\chi_1^0\to t\bar{t}$
($m_{1/2}\sim 400$ GeV). The diagrams involved in such a process contain contributions from $t$-
and $u$-channel exchange of stops, and from $s$-channel exchange of $Z$'s and pseudoscalar Higgs bosons.
The aforementioned threshold appears as a particular feature on the left-hand side plots:
An isolated detectable region for $m_{1/2}\sim 400$-$500$ GeV and $m_0\lesssim 300$ GeV
corresponding to the annihilation into a pair of real top quarks.

Larger values for the annihilation cross-section can be reached for higher values of $\tan\beta$.
In that case, the production process of a pair of down-type quarks (in particular $b\bar b$ pairs) and
charged leptons, dominates the total cross-section. In fact, the diagrams containing exchanges
of a pseudoscalar Higgs boson or a sfermion are enhanced by factors $\tan\beta$ and $1/\cos\beta$
respectively.
On the other hand, for high values of $\tan\beta$, the channels corresponding to
the annihilations into $W^+W^-$ and $t\bar{t}$ vanish. The first because of the reduction of the
coupling $\chi_1^0-\chi_i^\pm-W^\mp$; the second because of important destructive interference
between diagrams containing the exchange of a $Z$ boson and stops.

For the present scenario, the introduction of the NR operators gives rise to a very mild signature.
Actually, as in almost the whole parameter space the lightest neutralino is bino-like, its couplings
do not vary drastically. Moreover, the increment in the Higgs masses has a small impact on the
$\langle\sigma v\rangle$ factor. For indirect detection prospects, the main effect corresponds to a
slight increase in the LSP mass. Let us emphasize on the fact that, however, the detectable regions
are in the BMSSM case more cosmologically relevant than in the corresponding plain MSSM one.

Concerning figure \ref{gam1}, let us note that the
only astrophysical setup in which some useful information can be extracted
is the NFW$_c$ one. This means that in this scenario, in order to have some positive detection
in the $\gamma$-ray channel, there should exist some important enhancement of the signal by some
astrophysical mechanism (as the adiabatic contraction mechanism invoked in this
case). We note that, and this will be different from the case of antimatter signals, there is
however no important constraint on astrophysical boosts from the Galactic Center.
Gamma-ray detection does not rely, as is the case for positrons that we shall examine 
followingly, that much on local phenomena. 
In this respect, the NFW$_c$ results can be characterized as optimistic (it has been pointed
out that even by changing the gravitational collapse conditions, the results can get even more
pessimistic in the case, e.g., of a binary black hole formation in the GC), but not excluded.


\subsubsection{Light stops, heavy sleptons}
Figure \ref{gam2} presents the results for the second scenario with light stops and heavy sleptons.
\begin{figure}[tbp!]
\begin{center}
\vspace{-0.2cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gamB3-0.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gamB10-0.eps}\\
 \vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gamB3-1-0.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gamB10-1-0.eps}\\
 \vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gamB3-1-5.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/gamB10-1-5.eps}
\end{center}
% \vspace{-0.9cm}
\caption{{\footnotesize
Regions in the $[M_1,\,\mu]$ plane that can be detected by the
Fermi satellite mission for our scenario with light stops and heavy sleptons. 
The black lines depict the detectability regions for the corresponding halo profile assumptions 
and $5$ years of data acquisition: the area below the lines can be probed. The same applies
to lines forming closed regions with respect to the axes, as is the case for the NFW and NFW$_c$
profiles: the parameter space points lying in the interior of these regions yield signals that
are detectable.}}
\label{gam2}
\end{figure}
The experiment will be sensitive to the regions below/on the right of the contours.
Again, the detection prospects are maximised for low values of the $M_1$
and $\mu$ parameters, corresponding to light WIMPs.
However, the growth of any of the latter parameters gives rise to the opening of some production
channels, enhancing significantly the neutralino self-annihilation cross-section.
The first one appears for $m_\chi\sim m_Z/2$ and corresponds to the $s$-channel exchange
of a real $Z$ boson. 

The second one concerns the production channel of two real $W$ bosons. Once again, 
we notice the important difference in the detectability lines \textit{at} and right \textit{after} the
$h$ - pole region.
Let us note that in this scenario the neutralino LSP can be as heavy as
$\sim 110$ GeV, implying that the annihilation into a pair of top quarks is never kinematically allowed.

Finally, the region where $M_1\gg\mu$ is highly favored for indirect detection due to
the fact that the LSP is higgsino-like, maximising its coupling to the $Z$ boson. Let us recall
that the $Z$ boson does not couple to a pure gaugino-like neutralino. This feature appears as an
isolated region detectable by all three halo profiles in the right area of all plots. Unfortunately,
these regions are cosmologically disfavoured, as they yield too low a relic density.

Large values for the annihilation cross-section can be reached for high values of $\tan\beta$,
mainly because of the enhanced production of $b\bar b$ pairs.
On the other hand, for high values of $\tan\beta$, the threshold corresponding to the opening
of the annihilation into $W^+W^-$ is suppressed or enhanced for $\mu\gg M_1$ or $\mu\ll M_1$ respectively, 
due to the dependence of the $\chi_1^0-\chi_i^\pm-W^\mp$ coupling on the texture of the LSP.

For the present scenario, the introduction of the NR operators gives rise to an important
increase of the $\chi_1^0-\chi_1^0-A$ coupling when $\mu> M_1$, and therefore to a boost
in the annihilation into fermion pairs. On the other hand, as the Higgs boson $h$
becomes heavier, the processes giving rise to the final state $h\,Z$ get kinematically closed.

In the case presented in figure \ref{gam2}, there is a positive detection for all three halo profiles;
however, the regions that can be probed for either the NFW or the Einasto cases are cosmologically
irrelevant.

In fact, they could give rise to a positive detection near the $Z$-funnel and in the region where
the LSP is a higgsino state ($M_1\gtrsim 150$ GeV); nevertheless the first is already excluded by LEP
(at least for minimal scenarios) and the second generates too small a dark matter
relic density, below the WMAP limits.
On the other hand, the profile NFW$_c$ could test a large amount of the parameter space we examine,
particularly for high values of $\tan\beta$. Only the Higgs peak and the regions with a heavy LSP
escape from detection.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Positron detection}

\subsubsection{Correlated stop-slepton masses}
The results concerning the detectability perspectives for
the CMSSM-like scenario in the positron detection channel 
are quite pessimistic.
We already mentioned in our discussion of the singlet scalar model that
since the PAMELA and Fermi measurements, 
and according to our conservative treatment of considering the whole combined measurements as
the background for our study, the main issue in the positron channel is an
extreme domination of all measurements by a large background severely obscuring the signal.

One could invoke large boost factors of an astrophysical nature
as was the case in the first efforts to explain
the PAMELA excess through dark matter annihilations, a case in which a larger portion of the 
parameter space would be visible. However, it has been pointed out  
that it is highly unlikely to expect large boost factors due, e.g., to substructures
in the halo \cite{Lavalle:1900wn}. In this respect, if we assume a maximal clump-due signal enhancement 
by a factor $\sim 10$,  the only hope for positive detection of a non-LEP excluded area
might come for the bulk region, as it is the only one lying at the limits of detectability.
For the sake of brevity, we omit the relevant plots for the mSUGRA-like benchmark, since
no point of the parameter space can be tested.

We note that the considered background and AMS02 setup is exactly the same as in the singlet scalar
treatment presented in the previous chapter, with the data acquisition period being fixed at $3$ years.

\subsubsection{Light stops, heavy sleptons}
In figure  \ref{po2} we present the detection perspectives in the positron channel for our scenario
with light stops and heavy sleptons.
\begin{figure}[tbp!]
\begin{center}
\vspace{-0.2cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/poB3-0.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/poB10-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/poB3-1-0.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/poB10-1-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/poB3-1-5.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/poB10-1-5.eps}
\end{center}
% \vspace{-0.9cm}
\caption{{\footnotesize
Regions in the $[M_1,\,\mu]$ plane that can be detected by a $3$-year run of the 
AMS-02 satellite mission for the scenario with light stops and heavy sleptons, in the positron channel. 
The black lines depict the detectability regions for the $3$ considered propagation
models, MIN, MED and MAX: 
the parameter space points lying within the regions delimited by the black lines can be
probed, assuming the corresponding propagation models. 
Part of the mixed bino-higgsino region, as well as (marginally) some part of the $Z$ funnel
region can be probed.}}
\label{po2}
\end{figure}
The detectable parameter space regions lie within the zones delimited by the black lines
for the three propagation models: the oval-shaped blobs as well as the banana-shaped ones.
Once again, we notice the general features already present in the $\gamma$-ray channel.
The regions giving rise to a positive detection lie within the zone where the
LSP is a higgsino-like state, with mass $m_\chi>m_W$, in order to have the final state
$W^+W^-$ kinematically available. This region in general does not fulfill the WMAP limit.
However, and this is a novel feature of the BMSSM, with both $\epsilon_1$ and $\epsilon_2$
couplings turned on, a small region of the mixed higgsino-bino regime can be detected for
the MAX (and even the MED) propagation model. As we pointed out before, 
in this regime the total annihilation cross-section can be quite significantly enhanced, leading
to better detection perspectives.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Antiproton detection}
The last step in our analysis is to examine the antiproton channel predictions for the AMS02
experiment. We already mentioned the relevant experimental and background parameter values in
the singlet scalar model case. Once again, we stick to antiprotons with kinetic energies larger 
than $10$ GeV, whereas we consider that the AMS02 mission will collect data during three
years.

\subsubsection{Correlated stop-slepton masses}
In figure \ref{an1} we present our results for the detectability  of the BMSSM in comparison to
the CMSSM by the AMS-02 experiment for the antiproton channel. The detectable regions lie below the
black lines.
\begin{figure}[tbp!]
\begin{center}
%\vspace{-0.2cm}\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/an10-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/an10-1-0.eps}\hspace{0.2cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/an10-1-5.eps}
\end{center}
%\vspace{-0.9cm}
\caption{{\footnotesize
Regions in the $[m_0,\,m_{1/2}]$ plane that can be detected by a $3$-year run of the 
AMS-02 satellite mission for our mSUGRA-like scenario in the antiproton channel. 
The black lines depict the detectability regions for the $3$ considered propagation models: 
the area delimited by the axes and the black lines can be probed for the corresponding propagation
model (i.e. the region towards the lower left corner in each plot).}}
\label{an1}
\end{figure}
In the case $\tan\beta=3$, the experiment is not sensitive to any point in the parameter space satisfying also the
collider constraints and, hence, the corresponding results are once again omitted. 
A first remark here should concern the fact that the perspectives for antiproton detection are
significantly ameliorated with respect to the corresponding positron ones, at least for large values of $\tan\beta$.
We saw that this was also the case in the singlet scalar model of dark matter and attributed it to 
the important difference in background levels among the two channels.

Important areas of the viable parameter space are at the limits of detectability: the bulk region, but also, 
for some cases, part of the higgs funnel where sfermion exchange continues being efficient.
Now, as we stressed out before, the possible enhancements due for example to substructures are quite constrained.
Given however that some regions are marginally out of reach, it would not be impossible to state that 
even small boosts could render important (in a qualitative sense, due to their cosmological relevance) 
regions of the parameter space detectable by AMS-02.


\subsubsection{Light stops, heavy sleptons}
Figure \ref{an2} presents the results for antiprotons and for the second scenario under consideration.
AMS-02 will be able to probe the regions lying within the oval-like blobs and the banana-shaped regions
delimited by the black contours and the axes.
\begin{figure}[tbp!]
\begin{center}
\vspace{-0.2cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/anB3-0.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/anB10-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/anB3-1-0.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/anB10-1-0.eps}\\
\vspace{0.6cm}%\hspace{-2.5cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/anB3-1-5.eps}%\hspace{-2.3cm}
\includegraphics[width=5.5cm,angle=-90]{./susy/anB10-1-5.eps}
\end{center}
%\vspace{-0.5cm}
\caption{{\footnotesize
Regions in the $[M_1,\,\mu]$ plane that can be detected by a $3$-year run of the 
AMS-02 satellite mission for the scenario with light stops and heavy sleptons, in the antiproton channel. 
The black lines depict the detectability regions for the $3$ considered propagation models: 
the areas delimited by the axes and the black lines can be probed for the corresponding propagation
model (i.e. the regions towards the lower right side in each plot), as well as the areas delimited by closed
lines.}}
\label{an2}
\end{figure}



Once again, the BMSSM turns out to be more favorable for DM detection than the ordinary case
of light stops and heavy sleptons without NR operators.
Detectable regions fall either into the case of the higgsino-like neutralino regime, or in the
low-mass $Z$ funnel region. We point out that an important part of the area where the dark matter
relic density is fulfilled via coannihilation with the lightest stop could also be tested.
This last point might appear strange, since the coannihilation mechanism is inefficient at
present times. However, it should be noted that the detectable regions are mostly near the 
end of this region, where the correct relic density is in fact obtained through a 
combination of coannihilation and self-annihilation enhancement due to the mixed
gaugino - higgsino nature of the lightest neutralino.

An interesting remark concerns the different behaviour in the detectability lines among gamma-rays and
antiprotons just above the $h$ funnel. Whereas the opening of the gauge boson final state channels
lead to an important increase in the self-annihilation cross-section as well as the photon yield
at present times, this seems to be less the case for antiprotons. At this point, we should recall 
fig.\ref{antiprotonyieldmchi120GeV} that demonstrates that gauge boson final states are not the
most favourable ones for antiproton detection, since the corresponding yield is much lower 
compared to the hadronic one.


\subsection{Summarizing}
We saw that taking into account higher-dimensional contributions that could come from beyond the
MSSM physics can contribute significantly in resolving the little hierarchy problem. A very interesting
interplay appears with respect to dark matter phenomenology, since new regions yielding the
correct relic density appear and manage to evade collider constaints.

Dark matter detection gets quite challenged in this scenario, mainly due to the increase in mass
of practically the entire sparticle spectrum compared to the CMSSM case. The most promissing detection
mode appears to be the direct detection one, although interesting information could also come 
mainly from the gamma-ray and the antiproton channel. 

Especially concerning the last one, we see that important regions of the parameter space can
be probed. As an encouraging comment, we should again point out that the assumptions made in
this particular channel are quite conservative.

Overall, WIMP detection in this framework is best for small masses and when 
the neutralino obtains a significant higgsino component. On the other hand, resonnant
annihilation into a $h$ boson and then in fermion pairs is a mechanism that can be efficient 
in yielding large enough cross-sections and hence the correct relic density at early times
but is an inefficient mechanism at present times, since the relevant cross-section tends to
zero as $v \to 0$. This remark has already been made, for example, in \cite{Jungman:1995df} and is 
further explained in Appendix \ref{FeynmanGraphs}.









==> susy/susy.tex <==
\chapter{Supersymmetric solutions}

In the previous chapter we examined a really minimal way that tries to solve
the dark matter problem. We especially insisted on the fact that despite its
simplicity, the addition of just a singlet scalar in the theory can provide us
with a viable candidate for the missing matter content of the universe. We also 
saw that this candidate could be detected at present or oncoming 
experiments.

In this chapter we shall see how a dark matter candidate can arise within the context of
more complicated models. At first, we shall briefly describe some further issues that render the
Standard Model to be considered as a - probably - incomplete theory. Then, we shall see how 
an extension of the Poincar\'e symmetry that characterizes the SM lagrangian can provide us
with a framework that can actually solve these issues. Eventually, the same framework can, 
under certain assumptions, also give rise to a stable neutral particle that can answer the
dark matter question. Furthermore, we shall discuss how despite its elegance, the models
that can be constructed by virtue of this new extended symmetry, called supersymmetry (SUSY), 
are not without issues. This shall especially be the case for the simplest model
that can be constructed in this way, called the Minimal Supersymmetric Standard Model (MSSM).
Eventually, we shall discuss dark matter in a context that tries to resolve some of these
issues, focusing on two specific examples: one going beyond the MSSM framework (BMSSM)
and another one admitting non-minimal versions of the former. All of this shall, of course, 
be clarified much more in the following.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Some issues with the Standard Model...}
The Standard Model of particle physics is widely aknowldged as being extremely succesful in its predictions, 
both at a qualitative and a quantitative level. The new (at the time) particles it predicted have all been
discovered, and it could be said that it is really noteworthy that after the discovery of the 
top quark, its last missing ingredient before EWSB, for about 15 years no new major discovery has been made
pushing us to consider new physics from a strictly experimental point of view. Perhaps the two main experimental
issues that have arisen are neutrino oscillations, witnessing the existence of some non-zero neutrino masses, 
as well as the existence of dark matter, for which as we have said the Standard Model cannot account.
For the moment, its only missing ingredient is the mechanism breaking electroweak symmetry, or according
to our discussion until now the discovery of the higgs boson. 

However, there are reasons to think that despite its success the Standard Model should probably not be the 
ultimate theory. We have of course already mentioned that the Standard Model is a renormalizable theory that
can be in principle extrapolated up to arbitrarily high energies. It is nevertheless quite reasonable 
to wonder what happens if it is not treated in this way, but it is instead taken to be just
the low-energy limit of some higher theory.

If this is the case, an important issue arises. It is known that every renormalization procedure
intrinsically introduces some cut-off scale, say $\Lambda$. If one just considers the pure Standard Model,
then at the end of this procedure the cut-off should be sent to infinity and finite results should be acquired.
This is actually the case for the Standard Model: it is a renormalizable theory. But if we instead accept that
the Standard Model has some specific region of validity, then the cut-off cannot be sent to arbitrarily high 
scales. This argument leads to one of the main concerns indicating that the SM needs some ultraviolet 
completion from a more fundamental theory, as we shall see in the following paragraph.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The hierarchy problem}
In fig.\ref{fig:Higgs1loop} we show two examples of one-loop contributions to the higgs propagator, leading
to a redefinition of its physical mass according to usual renormalization procedures. 

\begin{figure}[ht]
\begin{center}
\includegraphics[width = 8cm]{./susy/HiggsHierarchy.eps}
\caption{{\footnotesize
Some 1-loop radiative corrections to the higgs boson mass.}}
\label{fig:Higgs1loop}
\end{center}
\end{figure}

To a good approximation (which shall be justified in a moment), one can ignore the light quark
loop contributions and only keep the one coming from the top quark. Then, the 
higgs mass receives corrections like
\begin{equation}
 \delta_{m_h}^2 = \frac{3 \Lambda^2}{8 \pi^2 u^2} 
\left[ \left( 
4 m_t^2 - 2 M_W^2 - M_Z^2 - m_h^2) + {\cal{O}}\left( \log \frac{\Lambda}{\mu}\right)
\right) \right]
\label{higgs1loopSM}
\end{equation}
where it can be seen that since fermion loop contributions scale as $m_f^2$, those coming from top quark 
loops are largely dominant. From eq.\eqref{higgs1loopSM} we can see that the standard model higgs mass
receives corrections depending both logarithmically \textit{and} quadratically on the cutoff scale.
Logarithmic corrections are actually not that large, since even if we replaced the cutoff scale by the
Planck mass, where gravity is generally expected to manifest its quantum nature (hence rendering the theory
incomplete), then the corresponding contributions are numerically quite small. This is not at all the case,
however, for the quadratic corrections. There is, thus, a natural tendency for the higgs mass to be pushed
towards the highest energy scale of the theory.

On the other hand, we expect that the higgs mass should lie somewhere around the electroweak scale. This is not
only due to that ``logically'' it should be somewhere around the scale where electroweak symmetry breaking
takes place. It is also a requirement coming from a series of bounds, such as the triviality and vacuum stability
ones. Of course, one could argue that since there are both positive and negative contributions to the quadratic
terms, there could be some important cancellation among them. This calculation has been demonstrated to be
a viable solution, it requires though very precise cancellations among very large quantities in order to 
yield very small ones. This effect is usually referred to as \textit{fine tuning}, whereas the resulting
problem is known as the ``hierarchy problem`` \cite{I-hierarchie}. It would be more ``natural''
to think of a mechanism that precisely eliminates the quadratic divergencies or largely supresses them. For the moment,
we just note that the usual way of eliminating terms in lagrangians, perturbative expansions etc is the 
introduction of symmetries: the gauge symmetry ``protects'' gauge bosons from receiving quadratically divergent
contributions, whereas chiral symmetry does so for the case of fermions. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Gauge coupling unification}
The Standard Model, appart from its endurance against experimental tests, is also a framework that allows
us to incorporate in the same lagrangian three out of the four fundamental forces in nature: the strong, 
weak and electromagnetic interactions. This unification is however incomplete. QCD on the one hand is just
a multiplicative factor for the electroweak sector, whereas even in the latter there are two distinct
gauge group factors resulting to two coupling constants.

This of course is by no means an original remark. Since the very early days of the standard model, a great
amount of research has been devoted to whether it would be possible to conceive a model with a simpler
gauge structure, perhaps based on a single semi-simple lie group, that can simultaneously describe all
three fundamental interactions (gravity is a bit more ambitious for our purposes). Schematically,
one can imagine a large gauge group, having $SU(3) \times SU(2) \times U(1)$ as one of its subgroups, 
breaking down at some scale in order to yield the SM along with some new matter and gauge bosons, 
which would probably be heavier than the ones we know.

This point of view was encouraged by the findings of the LEP collider at CERN, at which a precise 
measurement of the three coupling constants was possible. 
The evolution of the coupling constants is described by the renormalization group equations. 
Setting $t = \ln \mu$, the general one-loop
form of the beta function $\beta_a$ associated to a generic group's coupling constant $g_a$ is
\begin{equation}
 \beta_a \equiv \frac{dg}{dt} = 
\frac{g_a^3}{16 \pi^2} 
\left( \sum_i l(R_i) - 3 C_2 (G) \right)
\label{RGEgeneral}
\end{equation}
where the summation is over the irreducible representations of the group $G$, $l(R_i)$ is the 
Dynkin index of the representation $R_i$ and $C_2 (G)$ is the quadratic Casimir of the adjoint
representation of $G$. In the case of the standard model, this expression becomes
\begin{equation}
 \beta_a = \frac{1}{16\,\pi^2}\,b_a\,g_a^3,
\end{equation}
with the $b_a$ coefficients being
\begin{equation}
\left(b_1,\,b_2,\,b_3\right)=(41/10,\,-19/6,\,-7)
\end{equation}
and the normalization of $g_1$ being chosen according to the one imposed by unification conditions
as the ones found in $SU(5)$. Then, it is customary to also define $\alpha_a\equiv g_a^2/(4\,\pi)$.
The evolution of $1/\alpha_a$'s can be 
seen in fig.\ref{unif-SM} taken from ref.\cite{Martin:1997ns}.

\begin{figure}[ht]
\begin{center}
\includegraphics[width = 8cm]{./susy/unif-SM.eps}
\caption{{\footnotesize
Two-loop renormalization group evolution of the Standard Model gauge couplings. Figure taken from \cite{Martin:1997ns}.}}
\label{unif-SM}
\end{center}
\end{figure}
In this figure, starting from the LEP and LEP2 measurements, it has been rendered possible to compute
the predicted behaviour of the SM gauge coupling constants at high energy scales. Very soon it was
understood that the three coupling constants have a manifest tendency to unify at a high energy scale, 
roughly from $10^{12}$ up to $10^{16}$ GeV. This tendency, although it could also clearly be an accident,
is however an important element supporting the idea of unification. It turns out however that the three
couplings do not exactly meet. Unification is incomplete within the framework of the Standard Model.

Supersymmetry (SUSY) (see, for example, \cite{Wess:1992cp, Bailin:1994qt, Mohapatra:1986uf, Martin:1997ns, Drees:1996ca}), 
and especially its low-energy variant, is perhaps the most popular way of addressing and
resolving the hierarchy and unification issues. 
In the following paragraphs we shall introduce the basic formalism needed and
see how SUSY can stabilize the higgs mass and induce gauge coupling unification. Furthermore, we shall
focus on the solution SUSY can provide to the dark matter issue and examine the detection prospects
for one of the DM candidates appearing in supersymmetric frameworks, the lightest neutralino.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Elements of SUSY formalism}
\subsection{Supersymmetric algebra and superspace}
The $S$ matrix describing transitions from one quantum state to another, posesses a certain number of
symmetries. In particular:
\begin{enumerate}
 \item It is invariant under the action of the elements of the Poincar\'e group, whose generators
are the tranlsations and the Lorentz rotations $P_\mu$ and $M_{\mu\nu}$ respectively. These obey the
commutation relations
\begin{eqnarray}
\left[P_\mu,P_\nu\right]&=&0,\nonumber\\
\left[P_\mu,M_{\rho\sigma}\right]&=&i\,(\eta_{\mu\rho}\,P_\sigma-\eta_{\mu\sigma}\,P_\rho),\\
\left[M_{\mu\nu},M_{\rho\sigma}\right]&=&i\,(\eta_{\nu\rho}\,M_{\mu\sigma}-\eta_{\nu\sigma}\,M_{\mu\rho}-\eta_{\mu\rho}\,M_{\nu\sigma}+\eta_{\mu\sigma}\,M_{\nu\rho}).\nonumber
\end{eqnarray}
where $\eta_{\mu\nu}$ is the flat metric tensor.
 \item It is invariant under internal symmetries associated to some conserved quantum number (current)
according to Noether's theorem, such as the color, the electric charge etc. The generators of these
internal symmetries, say $T^a$, are Lorentz scalars and form Lie groups satisfying the relations
\begin{eqnarray}
\left[T^a,P_\mu\right]&=&0\nonumber\\
\left[T^a,M_{\mu\nu}\right]&=&0\\
\left[T^a,T^b\right]&=&i\,C^{abc}\,T^c\nonumber
\end{eqnarray}
where $C^{abc}$ are the group's structure constants.
\end{enumerate}
In 1967 Coleman and Mandula demonstrated a famous no-go theorem \cite{Coleman:1967ad} stating that apart from the Poincar\'e
group generators, the only conserved quantities in a local relativistic QFT with a mass gap can be a finite
number of Lorentz scalars associated with a Lie algebra of a compact Lie group 
(like the ones associated with the internal symmetries described above). This statement is valid if the theory
only contains commutators. In 1975, Haag, Lopuszanski and Sohnius demonstrated however that this restriction
can be evaded if one also includes anticommutators in the theory. Furthermore, they demonstrated that
the resulting extended Lie algebra (called \textit{supersymmetric algebra}) is the only one compatible 
with the symmetries of the $S$ matrix.

The most general supersymmetric algebra must contain the Poincar\'e group generators $P_\mu$ and $M_{\mu\nu}$
as well as a number $N$ of generators $Q^A$. It can be demonstrated that $N$ cannot
take arbitrary values, but should instead be $1, 2$ or $4$ in the case of global sypersymmetry, or also
$8$ in the case of local supersymmetry. Despite the theoretical interest of theories with $N > 1$ 
(for example $N = 4$ SYM theories posess the maximal possible symmetry compatible with global supersymmetry
and are finite, i.e. their beta functions vanish; extended supersymmetry plays an important role in some
string constructions), since quite some time it has been known that they result
to non-chiral fermions. In this work, we shall hence only focus on $N = 1$ theories.
\\ \\
The algebra of the generators is \cite{Wess:1974tw}
\begin{eqnarray}\label{algebre}
\{\qa,\qbb\}&=&2\,\sigma^\mu_{\alpha\dot{\beta}}\,P_\mu,\nonumber\\
\{\qa,\qb\}&=&\{\qba,\qbb\}=0,\nonumber\\
\left[\qa,P_\mu\right]&=&\left[\qba,P_\mu\right]=0,\\
\left[\qa,M_{\mu\nu}\right]&=&\frac{1}{2}\,(\sigma_{\mu\nu})_\alpha^\beta\,\qb,\nonumber\\
\left[\qba,M_{\mu\nu}\right]&=&-\frac{1}{2}\,\qbb\,(\sigma_{\mu\nu})_{\dot{\alpha}}^{\dot{\beta}}.\nonumber
\end{eqnarray}
where the matrices $\sigma_{\mu\nu}\equiv\frac{1}{4}\,(\sigma_\mu\bar{\sigma}_\nu-\sigma_\nu\bar{\sigma}_\mu)$
are the generators of the special linear group of $2\times2$ complex matrices with unit determinant, $SL(2,\mathbb{C})$.
The first equation further shows us that the mass dimension of the $Q$ generators must be $1/2$.
The operators $Q_\alpha$ and $\bar{Q}_\alpha$ are Weyl spinors belonging to the representations 
$(1/2, 0)$ and $(0, 1/2)$ of the Lorentz group. Conventionnally, we say that the former transforms as 
a left-handed Weyl spinor whereas the latter as a right-handed one.

An infinitesimal supersymmetric transformation of a field $\phi$ can be written by virtue of
two grassman variables $\theta$ and $\bar{\theta}$ as
\begin{equation}
\delta_\xt\,\phi=(\ta\,\qa+\bar{\theta}_{\dot{\alpha}}\,\bar{Q}^{\dot{\alpha}})\,\phi.
\end{equation}

Now, since we are extending the symmetries of the $S$ matrix, it can be convenient to also introduce some
sort of ``extended'' space, called \textit{superspace}. Superspace in $N = 1$ supersymmetry
is described by the four usual spacetime coordinates
along with two Grassmann variables $\ta$ and $\tba$ which obey the anticommutation relations
 \begin{equation}
 \{\ta,\tb\}=\{\tba,\tbb\}=\{\ta,\tbb\}=0.
 \end{equation}
A global (non - position - dependent) supersymmetric transformation in superspace is then defined 
by ``exponentiation'' of the infinitesimal transformation as 
 \begin{equation}\label{transsusy}
 G(x^\mu,\xt,\bt)=\exp[i\,(-x^\mu\,P_\mu+\xt\,Q+\bt\,\bar{Q})].
 \end{equation}
where it is assumed that $\xt$ and $\bt$ are of dimension  $-1/2$.
The composition of two supersymmetric transformations in superspace is written as
\begin{equation}
G(x^\mu,\xt,\bt)\,G(y^\mu,\zeta,\bar{\zeta}) =
G(x^\mu+y^\mu+i\,\zeta\,\sigma^\mu\bt-i\,\xt\,\sigma^\mu\bar{\zeta},\xt+\zeta,\bt+\bar{\zeta}).
\end{equation}
In particular, the composition of two supersymmetric transformations one of which does not modify 
spacetime is 
\begin{equation}\label{g0g}
G(0,\zeta,\bar{\zeta})\,G(x^\mu,\xt,\bt)=G(x^\mu+i\,\xt\,\sigma^\mu\bar{\zeta}-i\,\zeta\,\sigma^\mu\bt,\xt+\zeta,\bt+\bar{\zeta}).
\end{equation}
Eq. \eqref{g0g} allows us to define a differential representation of the $\qa$ and $\qba$ operators, as
\begin{eqnarray}
\qa&=&\frac{\partial}{\partial\ta}-i\,(\sigma^\mu)_{\alpha\dot{\alpha}}\,\tba\,\partial_\mu,\nonumber\\
\qba&=&\frac{\partial}{\partial\tba}-i\,\ta\,(\sigma^\mu)_{\alpha\dot{\alpha}}\partial_\mu,
\end{eqnarray}
where $P_\mu\equiv -i\,\partial_\mu$.
Then, it is further possible to define covariant derivatives as
\begin{eqnarray}
\da&=&\frac{\partial}{\partial\ta}+i\,(\sigma^\mu)_{\alpha\dot{\alpha}}\,\tba\,\partial_\mu,\nonumber\\
\dba&=&-\frac{\partial}{\partial\tba}-i\,\ta\,(\sigma^\mu)_{\alpha\dot{\alpha}}\partial_\mu.
\end{eqnarray}
We should note that the supercharges and the covariant derivatives anticommute
\begin{equation}
\{D,Q\}=\{\bar{D},Q\}=\{D,\bar{Q}\}=\{\bar{D},\bar{Q}\}=0.
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Superfields}
In a similar manner as we define fields as functions of spacetime, we can also define superfields $f(x,\xt,\bt)$ 
as functions of superspace. A superfield can in general be expanded in powers of $\xt$ and $\bt$.
This series cannot reach an arbitrarily high order, since the square of a grassmann variable is zero
\begin{eqnarray}\label{schamp}
f(x,\xt,\bt)&=&z(x)+\xt\,\phi(x)+\bt\,\bar{\chi}(x)+\xt\xt\,m(x)+\bt\bt\,n(x)\nonumber\\
&+&\xt\,\sigma^\mu\,\bt\,A_\mu(x)+\xt\xt\bt\,\bar{\lambda}(x)+\bt\bt\xt\,\psi(x)+\xt\xt\bt\bt\,d(x),
\end{eqnarray}
with $\xt\xt\equiv\xt^a\,\xt_a=\xt^a\,\epsilon_{ab}\,\xt^b$ 
and $\bt\bt\equiv\bt_{\dot a}\,\bt^{\dot a}=\bt_{\dot a}\,\epsilon^{\dot a\dot b}\,\bt_{\dot b}$, 
where $\epsilon$ is an antisymmetric tensor defined as $\epsilon^{12}= \epsilon_{21}=1$.

A clarification is in order: the superfield $f$ should not be taken as a physical field, corresponding
to one specific particle. It is just a function of superspace, whose components form a \textit{supermultiplet}.
The components, on the other hand, can actually have physical meaning.

Now, $f$ contains both bosonic components, ($z$, $m$, $n$, $A_\mu$, $d$) as well as fermionic
ones ($\phi$, $\chi$, $\lambda$, $\psi$). The dimension of $z$ is the same as the superfield's $f$ one.
The dimensions of the other fields augment progressively with powers of $\xt$ and $\bt$ up to the
value $[f]+2$ for the field $d$.

The most general superfield as defined in \eqref{schamp} is a reducible representation of
the supersymmetry algebra. Next, it would be useful to construct the irreducible representations
by imposing conditions on $f$.

\subsubsection{The chiral superfield}
The chiral superfield takes its name by the chiral nature of the SM fermions. Since for chiral
fields their left- and right - handed components are independent, the superfield describing them 
should need two degrees of freedom in order to fully describe them. Left-handed chiral superfields 
$\Phi$ are defined as 
\begin{equation}\label{defchi}
\dba\Phi=0.
\end{equation}
If we define a bosonic coordinate $y^\mu\equiv x^\mu+i\xt\sigma^\mu\bt$, 
we notice that $\dba y^\mu=\dba\xt=0$. Hence, the chiral superfield can be written as
\begin{equation}\label{schampchi}
\Phi(y,\xt)=z(y)+\sqrt{2}\,\xt\,\psi(y)+\xt\xt\,F(y).
\end{equation}
If $\Phi$ is of dimension $1$, $z$ must be a physical complex scalar field, 
$\psi$ a left-handed Weyl spinor and $F$ and auxiliary field of dimension $2$.
Eq. \eqref{schampchi} can be written as
\begin{eqnarray}
\Phi(x,\xt,\bt)&=&z(x)+i\,\xt\sigma^\mu\bt\,\partial_\mu\,z(x)+\frac{1}{4}\,\xt\xt\bt\bt\,\square\,z(x)\nonumber\\
&+&\sqrt{2}\,\xt\,\psi(x)-\frac{i}{\sqrt{2}}\,\xt\xt\,\partial_\mu\psi(x)\,\sigma^\mu\,\bt+\xt\xt\,F(x).
\end{eqnarray}
It can further be demonstrated that the product of two chiral fields is a chiral field. In particular, 
the components $\xt\xt$ are invariant under SUSY transformations. They transform as a total derivative
\begin{eqnarray}\label{int}
\left.\Phi_i\,\Phi_j\right|_{\xt\xt}&=&z_i\,F_j+z_j\,F_i-\psi_i\,\psi_j,\\
\left.\Phi_i\,\Phi_j\,\Phi_k\right|_{\xt\xt}&=&z_i\,z_j\,F_k+z_k\,z_i\,F_j+z_j\,z_k\,F_i-\psi_i\,\psi_j\,z_k-\psi_k\,\psi_i\,z_j-\psi_j\,\psi_k\,z_i.\nonumber
\end{eqnarray}\s
\\ \\
In the same way as in eq. \eqref{defchi}, we can define right-handed antichiral superfields
satisfying
\begin{equation}
\da\Phi^\dagger=0.
\end{equation}
Hence
\begin{equation}
\Phi^\dagger(y^\dagger,\bt)=z^*(y^\dagger)+\sqrt{2}\,\bt\,\bar{\psi}(y^\dagger)+\bt\bt\,F^*(y^\dagger).
\end{equation}

The product of a chiral and an antichiral superfield posess an interesting property: their $\xt\xt\bt\bt$
component contains the kinetic terms of $z$ and $\psi$
\begin{equation}\label{kin}
\left.\Phi_i\,\Phi_j^\dagger\right|_{\xt\xt\bt\bt}=F_i\,F^*_j+z^*_i\,\square\,z_j-\frac{i}{2}\,(\psi_i\,\sigma^\mu\,\partial_\mu\,\bar{\psi}_j-\partial_\mu\,\psi_i\,\sigma^\mu\,\bar{\psi}_j).
\end{equation}
Furthermore, this component transforms as a total derivative under supersymmetric transformations, 
it is therefore SUSY - invariant.

Using expressions \eqref{kin} and \eqref{int} we can construct the most general renormalizable lagrangian
containing only chiral superfields
\begin{equation}\label{lchi}
\mathcal{L}=\left.\Phi_i^\dagger\,\Phi^i\right|_{\xt\xt\bt\bt}+\left[\lambda_i\,\Phi^i+\frac{m_{ij}}{2}\,\Phi^i\,\Phi^j+\frac{g_{ijk}}{2}\,\Phi^i\,\Phi^j\,\Phi^k+c.h.\right]_{\xt\xt}.
\end{equation}
The first factor corresponds to kinetic terms. The following terms correspond to the $\xt\xt$ component of the 
\textit{superpotential} $W$
\begin{equation}\label{spot}
W(\Phi^i)=\lambda_i\,\Phi^i+\frac{m_{ij}}{2}\,\Phi^i\,\Phi^j+\frac{g_{ijk}}{2}\,\Phi^i\,\Phi^j\,\Phi^k.
\end{equation}
An important remark is that the superpotential must be a holomorphic function of the superfields $\Phi^i$.
If we break it down to components, we can get the corresponding lagrangian
\begin{eqnarray}
\mathcal{L}&=&i\,\partial_\mu\,\bar{\psi}_i\,\bar{\sigma}^\mu\,\psi^i+F^*_i\,F^i+z^*_i\square\,z^i\\
&+&\left[\lambda_i\,F^i+m_{ij}\,\left(z^i\,F^j-\frac{1}{2}\,\psi^i\,\psi^j\right)+g_{ijk}\,\left(z^i\,z^j\,F^k-\psi^i\,\psi^j\,z^k\right)+c.h.\right].\nonumber
\end{eqnarray}
The auxiliary fields $F$ and $F^*$ can be integrated out by means of their equations of motion
\begin{equation}
\frac{\partial\,\mathcal{L}}{\partial\,F^*}=0\qquad\text{et}\qquad\frac{\partial\,\mathcal{L}}{\partial\,F}=0
\end{equation}
which gives us an expression for $\mathcal{L}$ containing only the dynamical fields $z$ and $\psi$
\begin{equation}
\mathcal{L}=i\,\partial_\mu\,\bar{\psi}_i\,\bar{\sigma}^\mu\,\psi^i+z^*_i\square\,z^i+\frac{1}{2}\,\left(\frac{\partial^2\,W}{\partial\,z^i\,\partial\,z^j}\,\psi^i\,\psi^j+c.h.\right)-\mathcal{V}(z,z^*),
\end{equation}
where $\mathcal{V}(z,z^*)\equiv F^*_i\,F^i$ is the scalar potential.
This potential is manifestly positive: this is a consequence of sypersymmetry. Its minimum
corresponds to $F^i\geq 0$.


\subsubsection{The vector superfield}
In order to describe the SM gauge bosons now, we introduce the vector superfields defined by their 
self-conjugation condition
\begin{equation}
V(x,\xt,\bt)=V^\dagger(x,\xt,\bt).
\end{equation}
In terms of components, according to eq. \eqref{schamp}, a vector superfield is written as
\begin{eqnarray}
V(x,\xt,\bt)&=&C(x)+i\,\xt\,\chi(x)-i\,\bt\,\bar{\chi}(x)-\xt\,\sigma^\mu\,\bt\,v_\mu(x)\nonumber\\
&+&\frac{i}{2}\,\xt\xt\,\left[M(x)+i\,N(x)\right]-\frac{i}{2}\,\bt\bt\,\left[M(x)-i\,N(x)\right]\nonumber\\
&+&i\,\xt\xt\bt\,\left[\bar{\lambda}(x)+\frac{i}{2}\,\bar{\sigma}^\mu\,\partial_\mu\,\chi(x)\right]-i\,\bt\bt\xt\,\left[\lambda(x)+\frac{i}{2}\,\sigma^\mu\,\partial_\mu\,\bar{\chi}(x)\right]\nonumber\\
&+&\frac{1}{2}\,\xt\xt\bt\bt\,\left[D(x)+\frac{1}{2}\,\square\,C(x)\right];
\end{eqnarray}
where the fields $C$, $M$, $N$, $D$ and $v_\mu$ are real.
We should notice that the vector superfield is gauge invariant. The number of
degrees of freedom can be significantly reduced through gauge fixing. The Wess-Zumino gauge \cite{Wess:1974jb} is
a generalization of the usual unitary gauge and has the form
\begin{equation}\label{jwz}
V\rightarrow V+\Phi+\Phi^\dagger;
\end{equation}
where $\Phi$ is a non-physical chiral superfield that can be adjusted to eliminate $C$, $M$, $N$ and $\chi$.
This choice of gauge also implies that the fields $\lambda$ and $D$ are gauge-invariant, and that the vector
$v_\mu$ transforms as in the non-supersymmetric case:
\begin{equation}
v_\mu\rightarrow v_\mu-i\,\partial_\mu\,(z-z^*).
\end{equation}
\\ \\
So, in this gauge the vector superfield takes the form
\begin{equation}
V(x,\xt,\bt)=
-\xt\,\sigma^\mu\,\bt\,v_\mu(x)+
i\,\xt\xt\bt\,\bar{\lambda}(x)-i\,\bt\bt\xt\,\lambda(x)+
\frac{1}{2}\,\xt\xt\bt\bt\,D(x).
\end{equation}
This superfield is comprised of a gauge field $v_\mu$, a gaugino $\lambda$ and an auxiliary real field $D$.
The field strength tensor (which would be the equivalent of the usual 
$F^{\mu\nu}=\partial_\mu\,A_\nu-\partial_\nu\,A_\mu$)
is defined by means of gauge-invariant spinor fields
\begin{eqnarray}\label{vcin}
W_\alpha&=&-\frac{1}{4}\,\bar{D}\bar{D}D_\alpha\,V,\nonumber\\
\bar{W}_{\dot{\alpha}}&=&-\frac{1}{4}\,DD\bar{D}_{\dot{\alpha}}\,V.
\end{eqnarray}
We note that $\bar{D}_{\dot{\alpha}}\,W_\alpha=0$ and $D_\alpha\,\bar{W}_{\dot{\alpha}}=0$, 
which means that these fields are chiral and anti-chiral respectively.
In terms of components, we have
\begin{eqnarray}
W_\alpha&=&-i\,\lambda_\alpha(y)+\xt_\alpha\,D(y)-\frac{i}{2}
\,(\sigma^\mu\,\bar{\sigma}^\nu\,\xt)_\alpha\,v_{\mu\nu},\nonumber\\
\bar{W}_{\dot{\alpha}}&=&i\,\bar{\lambda}_{\dot{\alpha}}(y^+)+\bt_{\dot{\alpha}}\,\bar{D}(y^+)+
\frac{i}{2}\,(\sigma^\mu\,\bar{\sigma}^\nu\,\bt)_{\dot{\alpha}}\,v_{\mu\nu},
\end{eqnarray}
where $v_{\mu\nu}\equiv\partial_\mu v_\nu-\partial_\nu v_\mu$.
Since $W_\alpha$ is a chiral field, the component $\xt\xt$ of $W^\alpha\,W_\alpha$,
\begin{equation}
\left.W^\alpha\,W_\alpha\right|_{\xt\xt}=-2\,i\,
\lambda\,\sigma^\mu\,\partial_\mu\,\bar{\lambda}-
\frac{1}{2}\,v^{\mu\nu}\,v_{\mu\nu}+
\frac{i}{4}\,\epsilon^{\mu\nu\rho\sigma}\,v_{\mu\nu}\,v_{\rho\sigma},
\end{equation}
is SUSY-invariant, since it transforms as a total derivative.

From this last expression, we can construct the most general renormalizable lagrangian containing only 
vector superfields
\begin{eqnarray}\label{lvec}
\mathcal{L}&=&\frac{1}{4}\,\left(\left.W^\alpha\,W_\alpha\right|_{\xt\xt}+\left.\bar{W}_{\dot{\alpha}}\,\bar{W}^{\dot{\alpha}}\right|_{\bt\bt}\right)\nonumber\\
           &=&\frac{1}{2}\,D^2-i\,\lambda\,\sigma^\mu\,\partial_\mu\,\bar{\lambda}-\frac{1}{4}\,v^{\mu\nu}\,v_{\mu\nu}.
\end{eqnarray}
where the auxiliary field $D$ can be eliminated by means of its equations of motion. This field
will also contribute to the scalar potential, without modifying its positivity.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Interactions and supersymmetry breaking}
\subsubsection{Interactions}
Having so far examined theories with pure chiral or vector superfields, we can now construct 
a supersymmetric gauge - invariant lagrangian describing interactions among chiral superfields $\Phi_i$ 
and vector superfields $V$.
\\ \\
Under the action of a non-abelian group $G$, a chiral superfield transforms as
\begin{equation}\label{tcin}
\Phi^i\rightarrow(e^{-i\,\Lambda})^i_j\,\Phi^j,\qquad\Phi^\dagger_i\rightarrow\Phi^\dagger_j\,(e^{i\,\Lambda^\dagger})^j_i,
\end{equation}
where $\Lambda^i_j\equiv (T^a)^i_ j\,\Lambda_a(x,\xt,\bt)$ is defined in terms of chiral superfields $\Lambda_a$.
The matrices $T^a$ are hermitian generators of $G$ in the representation in which $\Phi$ lives. In particular, 
in the adjoint representation
\begin{eqnarray}
Tr\left(T^a\,T^b\right)&=&C(r)\,\delta^{ab},\nonumber\\
\left[T^a,T^b\right]&=&i\,f^{abc}\,T^c.
\end{eqnarray}
Since the transformation law for the chiral superfield is \eqref{tcin}, the kinetic term $\Phi^\dagger_i\,\Phi^i$
appearing in the lagrangian \eqref{lchi} is no longer gauge - invariant.
However, if we generalize the transformation law of $V$, eq. \eqref{jwz}, for non-abelian groups as
\begin{equation}
e^V\rightarrow e^{-i\,\Lambda^\dagger}\,e^V\,e^{i\,\Lambda},
\end{equation}
we can construct a SUSY-invariant kinetic term as
\begin{equation}
\left.\Phi^\dagger_i\,\left(e^V\right)^i_j\,\Phi^j\right|_{\xt\xt\bt\bt}.\\
\end{equation}
\\ \\
The field strength tensor \eqref{vcin} for non abelian interactions must then be redefined as
\begin{eqnarray}
W_\alpha=-\frac{1}{4}\,\bar{D}\bar{D}\,e^{-V}\,D_\alpha\,e^V \ , \
%\nonumber\\
\bar{W}_{\dot{\alpha}}=-\frac{1}{4}\,DD\,e^{-V}\,\bar{D}_{\dot{\alpha}}\,e^V.
\end{eqnarray}
These field strength tensors in their turn transform as
\begin{equation}
W_\alpha\rightarrow W^\prime_\alpha=e^{-i\,\Lambda}\,W_\alpha\,e^{i\,\Lambda}.
\end{equation}
The lagrangian for vector superfields is the same as in eq. \eqref{lvec}, appart from the fact
that a trace must be taken over gauge indices.

Then, the most general renormalizable lagrangian including gauge interactions among chiral and vector superfields
can be written as
\begin{eqnarray}
\mathcal{L}&=&\frac{1}{4\,C(r)}\,\left(\left.W^\alpha\,W_\alpha\right|_{\xt\xt}+\left.\bar{W}_{\dot{\alpha}}\,\bar{W}^{\dot{\alpha}}\right|_{\bt\bt}\right)+\left.\Phi^\dagger\,e^V\,\Phi\right|_{\xt\xt\bt\bt}\nonumber\\
&+&\left[\left.\left(\lambda_i\,\Phi^i+\frac{m_{ij}}{2}\,\Phi^i\,\Phi^j+\frac{g_{ijk}}{2}\,\Phi^i\,\Phi^j\,\Phi^k\right)\right|_{\xt\xt}+c.h.\right].
\end{eqnarray}


\subsubsection{Supersymmetry breaking}
A phenomenologically viable supersymmetric model should include terms breaking supersymmetry.
One possibility is that supersymmetry can be an exact symmetry of the theory, but which is spontaneously
broken by the vacuum choice. In this way, supersymmetry will not be manifest at low energies, especially
the electroweak scale which is of interest for us.
However, it turns out quite difficult to spontaneously break supersymmetry. 
% The definition of its
% algebra, equations \eqref{algebre}, implies that the Hamiltonian is defined in terms of the hypercharges
% \begin{equation}
% H=\frac{1}{4}\,\left(\qa\qba+\qba\qa\right).
% \end{equation}
% Supersymmetry is not broken once  $H|0\rangle=0$. This implies that the vacuum
% energy is zero. Inversely seen, if supersymmetry is broken spontaneously, the 
% vacuum state will have a positive energy. It can be demonstrated that SUSY is broken
% if $F_i$ or $D^a$ do not cancel in the vacuum. We thus search for models where the 
% equations $F_i=0$ and $D^a=0$ are not satisfied simultaneously.

There have been several proposals for spontaneous breaking of supersymmetry in the literature. 
These proposals always include new particles and interactions at some high energy scale.
The standard picture is that supersymmetry breaking occurs in some ``hidden sector'' which
does not communicate directly with the rest of the spectrum, the breaking being then ``mediated''
to the other parts of the Lagrangian through some \textit{messenger} sector.
The most well-known examples are gravity-mediated supersymmetry breaking \cite{Freedman:1976xh,Cremmer:1982en}, 
gauge-mediated breaking \cite{Giudice:1998bp}, anomaly-mediated breaking \cite{Randall:1998uk, Falkowski:2005ck}
or supersymmetry breaking induced by the existence of extra dimensions \cite{Quiros:2003gg}.
Combinations of these mechanisms can also be effective, often motivated by string constructions
\cite{Dudas:2008qf}.
However, there is no consensus on the mechanism that induces SUSY - breaking. It might be
that future experimental data shall help in this direction.

It is nonetheless possible to parametrize the effects of supersymmetry breaking at low
energies, introducing terms breaking it explicitly in the otherwise SUSY - invariant Lagrangian.
The new couplings must be \textit{soft}, so as to not reintroduce quadratic divergencies in the theory. 
In particular, we cannot introduce dimensionless couplings.

The most general renormalizable Lagrangian explicitly breaking supersymmetry, $\mathcal{L}_\text{soft}$
must include
\begin{itemize}
\item[\textbullet]  masses for the scalars $-m_{\phi_i}^2\,\left|\phi_i\right|^2$,
\item[\textbullet]  masses for the gauginos $-\frac{1}{2}\,m_{\lambda_i}\,\bar{\lambda}_i\lambda_i$,
\item[\textbullet]  trilinear scalar interactions $-A^{ijk}\,\phi_i\,\phi_j\,\phi_k+ c.h.$
\item[\textbullet]  bilinear scalar terms $-b^{ij}\,\phi_i\,\phi_j+c.h.$.
\end{itemize}

Fermionic terms could also in principle be included, but they can be absorbed by a 
redefinition of the superpontential, the scalar masses and the trilinear couplings.
We note that it has been rigorously demonstrated that a theory breaking supersymmetry
softly does not reintroduce quadratic divergencies in the perturbative expansion
\cite{Girardello:1981wz}.

The soft Lagrangian $\mathcal{L}_\text{soft}$ breaks supersymmetry, since it 
only contains scalars and gauginos without their superpartners. These soft terms
would induce a mass for the scalars and the gauginos, even in the absence of
mass terms for vector bosons and ordinary fermions.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Minimal Supersymmetric Standard Model}
\subsection{The MSSM}

The Minimal Supersymmetric Standard Model (MSSM)
\cite{Fayet:1976et,Fayet:1976cr,Fayet:1977yc,Nilles:1983ge,Martin:1997ns} 
is, as stated in its name, the simplest supersymmetric extension to the Standard Model.
It is minimal in the sense that it contains the smallest possible number of 
new fields.

The MSSM is based on the SM gauge group $\sut\times\sud\times
\uu$. Supersymmetry associates to every gauge boson a spin - $1/2$ fermion.
The gauge bosons belong to $8+3+1$ vector superfields, associated to the groups
$\sut$, $\sud$ and $\uu$. The superpatners of the gauge bosons are usually 
collectively called gauginos. In particular, the superpatners of the gluons are
called gluinos $\tilde g$, whereas the ones associated to the $W^\pm$, $W^3$ and
$B$ gauge bosons of the electroweak sector are called winos $\tilde W$ and 
binos $\tilde B$ respectively. In table \ref{svec} we indicate the quantum numbers
of the various vector superfields of the MSSM. As usually, the charge $Q_\text{em}$
associated with electromagnetism is given by the sum of the third component of the
isospin, $T_3$ and the hypercharge $Y$ of the particle.

\begin{table}[!h]
\centering
\begin{tabular}{|c||cc|ccccc|}
\hline
$\begin{array}{c}\mbox{Super-}\\\mbox{field}\end{array}$ & \multicolumn{2}{c|}{$\begin{array}{c}\mbox{Spin}\\1\qquad 1/2\end{array}$} & $\sut$ & $\sud$ & $T_3$ & $\uu$ & $Q_\text{em}$ \\
\hline\hline
$B$ & $B_\mu$ & $\tilde{B}$ & $1$ & $1$ & $0$ & $0$ & $0$ \\
$W$ & $\begin{array}{r}W_\mu^+\\W_\mu^3\\W_\mu^-\end{array}$ & $\begin{array}{r}\tilde{W}^+\\\tilde{W}^3\\\tilde{W}^-\\\end{array}$ & $1$ & $3$ & $\begin{array}{r}+1\\0\\-1\end{array}$ & $0$ & $\begin{array}{r}+1\\0\\-1\end{array}$ \\
$g$ & $g_\mu$ & $\tilde{g}$ & $8$ & $1$ & $0$ & $0$ & $0$ \\
\hline
\end{tabular}
\caption{Vector superfields of the MSSM}
\label{svec}
\end{table}

On the other hand, the matter content of the MSSM is described by chiral 
superfields. We follow the standard convention according to which the chiral
superfields are defined in terms of left-handed Weyl spinors, hence their charge
conjugates correspond to right-handed spinors. Two $\sud$ doublets ($Q_i$ and $L_i$) and three singlets 
($u^c_i$, $d^c_i$ and $e^c_i$) are needed to account for the different quarks and leptons.
The index $i=1,2,3$ corresponds to different fermion families. We note that
like the minimal SM, the MSSM does not contain right-handed neutrinos.

In the Standard Model, a single Higgs doublet field $H$ along with its conjugate is sufficient
to provide masses for all quarks and massive leptons.
In the MSSM, two Higgs doublets are instead necessary, often denoted as
$H_u$ and $H_d$. It is actually supersymmetry itself that imposes the introduction of
two doublets instead of one. This can be seen in two ways:

\begin{itemize}

\item In supersymmetry, the superpotential \eqref{spot} is, as we said, a holomorphic
function in the superfields it containts. Hence, a Higgs supermultiplet
with isospin $Y = +1/2$ cannot give rise to Yukawa couplings that generate masses
for down-type quarks. The inverse applies to a $Y = -1/2$ Higgs supermultiplet, 
which can only generate masses for up-type quarks. The holomorphic nature of the
superpotential obliges us hence to introduce two distinct Higgs doublet fields.

\item The Higgs superpatners, called higgsinos,  are expected (and actually \textit{do}) 
give rise to new contributions to the chiral anomaly. 
In order to achieve cancellation of these anomalies, one must have
\begin{equation}
\sum_\text{fermions}Y^3=\sum_\text{fermions}T_3^2\cdot Y=0.
\end{equation}
Now, whereas in the Standard Model the quark and lepton contributions cancel, 
in the MSSM case this is no longer valid. It is only after the introduction of
a second Higgs doublet that anomaly cancellation is actually achieved.
\end{itemize}

The chiral superfields and their quantum numbers are summarized in table \ref{schi}, which along
with table \ref{svec} sum up the particle content of the MSSM.

\begin{table}
\centering
\begin{tabular}{|c||cc|ccccc|}
\hline
$\begin{array}{c}\mbox{Super-}\\\mbox{field}\end{array}$ & \multicolumn{2}{c|}{$\begin{array}{c}\mbox{Spin}\\1/2\qquad 0\end{array}$} & $\sut$ & $\sud$ & $T_3$ & $\uu$ & $Q_\text{em}$ \\
\hline\hline
$Q$ & $\begin{array}{r}  u_L\\d_L\end{array}$ & $\begin{array}{r}  \tilde{u}_L\\\tilde{d}_L\end{array}$ & $3$ & $2$ & $\begin{array}{r}1/2\\-1/2\end{array}$ &  $1/6$ & $\begin{array}{r}2/3\\-1/3\end{array}$ \\
$u^c$ & $\bar{u}_R$ & $\tilde{u}_R^*$ & $\bar{3}$ & $1$ & $0$ & $-2/3$ & $-2/3$ \\
$d^c$ & $\bar{d}_R$ & $\tilde{d}_R^*$ & $\bar{3}$ & $1$ & $0$ &  $1/3$ &  $1/3$ \\
\hline
$L$ & $\begin{array}{r}\nu_L\\e_L\end{array}$ & $\begin{array}{r}\tilde{\nu}_L\\\tilde{e}_L\end{array}$ & $1$ & $2$ & $\begin{array}{r}1/2\\-1/2\end{array}$ & $-1/2$ & $\begin{array}{r}0  \\-1  \end{array}$ \\
$e^c$ & $\bar{e}_R$ & $\tilde{e}_R^*$ &       $1$ & $1$ & $0$ &    $1$ &    $1$ \\
\hline
$H_u$ & $\begin{array}{r}H_u^+\\H_u^0\end{array}$ & $\begin{array}{r}\tilde{H}_u^+\\\tilde{H}_u^0\end{array}$ & $1$ & $2$ & $\begin{array}{r}1/2\\-1/2\end{array}$ &  $1/2$ & $\begin{array}{r}1\\0 \end{array}$ \\
$H_d$ & $\begin{array}{r}H_d^0\\H_d^-\end{array}$ & $\begin{array}{r}\tilde{H}_d^0\\\tilde{H}_d^-\end{array}$ & $1$ & $2$ & $\begin{array}{r}1/2\\-1/2\end{array}$ & $-1/2$ & $\begin{array}{r}0\\-1\end{array}$ \\
\hline
\end{tabular}
\caption{The chiral superfields of the MSSM.}
\label{schi}
\end{table}

There is only one missing ingredient before writing down the MSSM Lagrangian density.
If supersymmetry where an exact symmetry, then every particle belonging to the same
supermultiplet would have the same mass as its supersymmetric partner. So, for example, 
there should exist selectrons $\tilde{e}_L$ and $\tilde{e}_R$ with masses $m_{\tilde e}=m_e\sim 0.51$ MeV.
However, it is quite apparent that if this was the case, such scalars should have been
observed. This means that if supersymmetry has anything to do with the physical world
at the electroweak scale, it must be broken.

The MSSM Lagrangian is thus comprised of two main pieces: The first
one is supersymmetric and contains all kinetic terms for chiral and vector superfields, 
as well as all terms that can be derived from the superpotential.
The second part contains all SUSY - breaking terms, which we argued should be soft.
So, we can write
\begin{equation}\label{mssm}
\mathcal{L}=\mathcal{L}_\text{kin}+\mathcal{L}_\text{W}+\mathcal{L}_\text{soft}.
\end{equation}
\\
Under the light of the previous discussion, the most general gauge-invariant superpotential of the MSSM is
\begin{eqnarray}\label{potentiel}
W=\sum_{i,j=1}^3\,\sum_{a,b=1}^2\left[\lambda^{ij}_u\,Q_{ai}\,\epsilon^{ab}\,H_{ub}\,u_j-\lambda^{ij}_d\,Q_{ai}\,\epsilon^{ab}\,H_{db}\,d_j\right.\nonumber\\
\left.-\lambda^{ij}_l\,L_{ai}\,\epsilon^{ab}\,H_{db}\,e_j+\mu\,H_{ua}\epsilon^{ab}\,H_{bd}\right].
\end{eqnarray}
where $\lambda_u$, $\lambda_d$ and $\lambda_l$ are complex $3\times 3$ matrices in
family space, corresponding to the Yukawa couplings, whereas the $\mu$ term
is a supersymmetric mass term for the Higgs doublets.
\\ \\
This superpontential is invariant under a discrete symmetry called $R$ - parity, defined as
\begin{equation}
R_p=(-1)^{2\,S+3\,(B-L)},
\label{Rparity}
\end{equation}
where $S$ is each particle's spin and $B$ and $L$ are the baryonic and leptonic numbers respectively.
$R$ - parity was first introduced to ensure baryon and lepton number conservation, 
so as to prevent rapid proton decay. Particles belonging to the same supermultiplet do not have
the same $R$ - parity: Standard Model particles have $R_p=1$, whereas their superpatners have
$R_p=-1$.
\\ \\
Appart from its initial motivation, $R$ - parity has very far-reaching consequences:
\begin{itemize}
\item  sparticles are forcedly produced in pairs.
\item  The Lightest Supersymmetric Particle (LSP) is completely stable.
\item  sparticles other than the LSP decay in an odd number of sparticles.
\end{itemize}

The structure of the MSSM Lagrangian is highly constraining for the parameters
it includes. However, the soft breaking terms generate a huge number of free
parameters. The relevant part of the Lagrangian is
\begin{eqnarray}\label{doux}
\mathcal{L}_\text{soft}=&-&\frac{1}{2}\left[M_1\,\tilde{B}\tilde{B}+\sum_{a=1}^3M_2\,\tilde{W}^a\tilde{W}_a+
\sum_{a=1}^8M_3\,\tilde{g}^a\tilde{g}_a+c.c.\right]\nonumber\\
&-&\sum_{i=1}^3\left[m_{\tilde{Q}_i}^2\,|\tilde{Q}_i|^2+m_{\tilde{L}_i}^2\,|\tilde{L}_i|^2+m_{\tilde{u}_i}^2\,
|\tilde{u}_i|^2+m_{\tilde{d}_i}^2\,|\tilde{d}_i|^2+m_{\tilde{e}_i}^2\,|\tilde{e}_i|^2\right]\nonumber\\
&-&m_{\tilde{H}_u}^2\,|\tilde{H}_u|^2-m_{\tilde{H}_d}^2\,|\tilde{H}_d|^2-(B\,\mu\sum_{a=1}^2\tilde{H}_u^a\,\tilde{H}_{da}+c.c.)\\
&-&\left[A_u^{ab}\,\tilde{Q}_{ai}\,\epsilon^{ij}\,\tilde{H}_{uj}\,\tilde{u}_b-A_d^{ab}\,\tilde{Q}_{ai}\,
\epsilon^{ij}\,\tilde{H}_{dj}\,\tilde{d}_b-A_e^{ab}\,\tilde{L}_{ai}\,\epsilon^{ij}\,\tilde{H}_{dj}\,\tilde{e}_b+c.c.\right].\nonumber
\end{eqnarray}
where in eq. \eqref{doux} $M_1$, $M_2$ and $M_3$ correspond to the masses of the bino, the winos and the gluinos respectively.
The terms in the second line correspond to the mass terms for squark and sleptons. In the third line, 
there are new contributions to the Higgs potential. Finally, the fourth line corresponds to trilinear couplings 
among three scalars. We note that the $A_{u,d,l}$ factors are $3\times 3$ complex matrices in 
family space.
\\ \\
After having presented some basic elements of formalism, we shall now see how supersymmetry (and, notably, the MSSM)
provides solutions to the Standard Model issues mentioned previously: the Higgs mass hierarchy problem, the
unification of gauge couplings, as well as the dark matter problem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{SUSY to the rescue!}
\subsubsection{Solution to the hierarchy problem}

Supersymmetry can offer a solution to the hierarchy problem discussed previously.
In the same way as gauge symmetry ``protects'' the masses of vector bosons and
chiral symmetry the ones of fermions from receiving quadratic divergencies, SUSY
protects the masses of scalars. We saw that the problem arose from the contributions
of fermion and gauge boson loop correction to the Higgs mass. It is well-known that
fermion loops allways carry an extra factor of $-1$ with
respect to the case where a boson ``circulates'' in the loop.

So, for example, if we suppose $N_S$ scalar particles of mass $m_S$ and with
trilinear and quartic couplings $v\,\lambda_S$ and $\lambda_S$ respectively, 
their $1$-loop contribution to the Higgs mass shall be of the form
\begin{equation}
\Delta\,M_H^2=\frac{N_S\,\lambda_S}{16\,\pi^2}\left[-\Lambda^2+2\,m_S^2\,\log\frac{\Lambda}{m_S}\right]
-\frac{N_S\,\lambda_S^2\,v^2}{16\,\pi^2}\left[-1+2\,\log\frac{\Lambda}{m_S}\right]+\mathcal{O}\left(\frac{1}{\Lambda^2}\right),
\end{equation}
which also contains quadratic divergencies.

However, if we suppose that the Higgs couplings to the scalar particles have some relation with its
couplings to fermions of the form $\lambda_f^2=-\lambda_S$, and that the number of bosonic and 
fermionic degrees of freedom is equal ($N_S=N_f$), 
the total radiative corrections induced by the presence of fermions and
scalars is
\begin{equation}
M_H^2 =m_H^2 + \frac{N_f\,\lambda_f^2}{4\,\pi^2} \left[(m_f^2-m_S^2)\,\log\frac{\Lambda}{m_S}+3\,m_f^2\,
\log\frac{m_S}{m_f}\right]+\mathcal{O}\left(\frac{1}{\Lambda^2}\right).
\end{equation}

At this point, we see that the quadratic divergencies have dissapeared.
We remark that logarithmic divergencies are still there, but as we said even
if the theory's cutoff is pushed to the Plank scale, these remain quite moderate.
An important remark is, though, that in order to have exact cancellation of
the quadratic divergencies a very strong condition is imposed, namely that
$m_S=m_f$. This last condition is however in straight contradiction to our
discussion so far, since we said that supersymmetry must be broken and that
sparticles should receive additional contributions with respect to their
SM counterparts if we wish for a phenomenologically viable theory.

This last point motivates electroweak scale supersymmetry: the superpatners
must not be much heavier than the corresponding SM particles, since this would
destabilize the Higgs boson mass once more. As we shall see in the following, 
even more complications may appear, concerning mostly the mass of the lightest
higgs boson, both from an experimental and a theoretical point of view.

\subsubsection{Gauge coupling unification}

Another point where the MSSM turns out to be successful is the unification of
coupling constants. The renormalization group equations for the three gauge couplings 
$g_1$, $g_2$ and $g_3$ are again given by eq. \eqref{RGEgeneral}, but this time
the coefficients $b_a$ are different than in the Standard Model case:
\begin{equation}
\left(b_1,\,b_2,\,b_3\right)=\left\{\begin{array}{l}(41/10,\,-19/6,\,-7)
\qquad\text{MS}\\(33/5,\,1,\,-3)\hspace{2.0cm}\text{MSSM.}\end{array}\right.
\end{equation}
\begin{figure}[!h]
\centering
\includegraphics[width=0.55\textwidth,clip=true]{./susy/unif-MSSM.eps}
\vspace*{-2mm}
\caption{\footnotesize{
Gauge coupling constant evolution in the MSSM. 
One and two loop corrections are included in the running. Figure taken from ref.\cite{Martin:1997ns}.
}}
\label{unificag-MSSM}
\vspace*{-3mm}
\end{figure}
The coefficients in the MSSM case are larger, due to the larger number of particles 
contributing to the beta-functions. In fig.\ref{unificag-MSSM} we can see a
comparison of the RGE evolution of the $\alpha_a^{-1}$'s, at two loops
in perturbation theory. Contrary to the Standard Model case, the MSSM contains
the right number of fields to ensure unification of the gauge couplings at some
large scale, called the Grand Unification scale $\mgut\sim 2\cdot 10^{16}$ GeV.
Unification of coupling constants at some scale could indicate the existence of 
some Grand Unified Theory (GUT) at the scale where the coupling constants acquire
the same value.

This is a further motivation for weak-scale supersymmetry: it has been
demonstrated that gauge coupling unification is not a general feature of supersymmetric
theories and models. In order to achieve it, the superpatner contributions must enter
the RGE running at a scale being sufficiently low so as to leave enough ``space'' for the
coupling constants to evolve in this way.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The physical particles of the MSSM}
Before setting off to examine dark matter in the framework of the MSSM, it is useful to discuss the
physical particle spectrum of the model, i.e. the mass eigenstates appearing in the Lagrangian. 
Tables \ref{svec} and \ref{schi} summarize the various gauge eigenstates of the model. We know
that after EWSB several particles of the Standard Model that are gauge eigenstates are no longer mass
eigenstates, since they appear in quadratic crossed terms in the Lagrangian. This is also the case
for the MSSM, with mixing effects being even more extended than in the SM. As a first remark, we note
that the SM particles' definitions are not altered at tree level (appart, of course, from the
Higgs sector). We shall now describe what happens
with the rest of the particle content. Our intention is not to provide a detailed description, but rather
to summarize a number of elements that shall be useful for the following, namely to just identify the
physical degrees of freedom.

\subsubsection{The Higgs fields}
We saw that in the MSSM two Higgs doublets are required, which we denote by $H_u \equiv H_2 = (H_2^+, H_2^0)^T$ 
and $H_d \equiv H_1 = (H_1^0, H_1^-)^T$. Upon EWSB, the neutral components of the two doublets acquire 
non-zero VEVs $v_1/\sqrt{2}$ and $v_2/\sqrt{2}$ for $H_1^0$ and $H_2^0$ respectively, with $(v_1 + v_2)^2 = 
v^2 = (246 \ \mbox{GeV})^2$. We further define the parameter
\begin{equation}
 \tan\beta = \frac{v_2}{v_1}
\end{equation}
As usually, the physical Higgs fields are obtained by expaning around the scalar potential's minimum
\begin{eqnarray}
 H_1 & = & (H_1^0, H_1^-)^T = \frac{1}{\sqrt{2}} (v_1 + H_1^0 + i P_1^0, H_1^-)^T\\ \nonumber
 H_2 & = & (H_2^+, H_2^0)^T = \frac{1}{\sqrt{2}} (H_2^+ , v_2 + H_2^0 + i P_2^0)^T
\end{eqnarray}
with the real parts corresponding to $CP$ - even higgs bosons and the imaginary parts to $CP$ - odd ones
and the goldstone bosons.

Then, the physical fields/mass eigenstates of the model can be expressed as linear combinations of the
gauge eigenstates, as follows:
\begin{itemize}
 \item First, we can write down the expression for the neutral goldstone boson and the $CP$ - odd  
Higgs
\begin{equation}
\left( \begin{array}{c}   G^0 \\ A \end{array} \right) 
= \left( \begin{array}{cc} \cos \beta & \sin \beta \\
- \sin \beta & \cos \beta \end{array} \right) \ 
\left( \begin{array}{c}   P_1^0 \\ P_2^0 \end{array} \right)
\end{equation}
 \item Then, we have the charged Goldstone bosons and the charged Higgses
\begin{equation}
\left( \begin{array}{c}   G^\pm \\ H^\pm \end{array} \right) 
= \left( \begin{array}{cc} \cos \beta & \sin \beta \\
- \sin \beta & \cos \beta \end{array} \right) \ 
\left( \begin{array}{c}   H_1^\pm \\ H_2^\pm \end{array} \right) 
\end{equation}
 \item Finally, we have the two physical $CP$ - even higgs bosons
\begin{equation}
\left( \begin{array}{c}   H \\ h \end{array} \right) 
= \left( \begin{array}{cc} \cos \alpha & \sin \alpha \\
- \sin \alpha & \cos \alpha \end{array} \right) \ 
\left( \begin{array}{c}   H_1^0 \\ H_2^0 \end{array} \right) 
\end{equation}
\end{itemize}
where $\alpha$ is a rotation angle. In principle, the higgs sector should contribute 
six new free parameters to the theory. It turns out however that there are several relations among
them, which amount to only two free parameters, often taken to be $\tan\beta$ and $M_A$.

\subsubsection{The sfermions}
Sfermions can also mix, since they share quantum numbers. The mass matrices have the general form
\begin{equation} 
\label{sqmass_matrix}
{\cal M}^2_{\tilde{f}} =
\left(
  \begin{array}{cc} m_f^2 + m_{LL}^2 & m_f \, X_f  \\
                    m_f\, X_f    & m_f^2 + m_{RR}^2 
  \end{array} \right) 
\end{equation}
where
\begin{equation}
\begin{array}{l} 
\ m_{LL}^2 =m_{\tilde{f}_L}^2 + (I^{3L}_f - Q_f s_W^2)\, M_Z^2\, c_{2\beta} \\\
m_{RR}^2 = m_{\tilde{f}_R}^2 + Q_f s_W^2\, M_Z^2\, c_{2\beta} \\\
\ \ X_f  = A_f - \mu (\tb)^{-2 I_f^{3L}} 
\label{mass-matrix}
\end{array}
\end{equation}
These mass matrices are diagonalized by means of $2 \times 2$ unitary matrices 
\begin{equation}
 R^{\tilde f} =  \left( \begin{array}{cc}
     c_{\theta_f} & s_{\theta_f} \\ - s_{\theta_f} & c_{\theta_f}
  \end{array} \right)  \ \ \ \ , \ \ c_{\theta_f} \equiv \cos \theta_{\tilde f} 
\ \ {\rm and} \ \ s_{\theta_f} \equiv \sin \theta_{\tilde f}
\end{equation}
The mixing angle and sfermion masses are then given by 
\begin{equation}
s_{2\theta_f} = \frac{2 m_f X_f} { m_{\tilde{f}_1}^2
-m_{\tilde{f}_2}^2 } \ \ , \ \ 
c_{2\theta_f} = \frac{m_{LL}^2 -m_{RR}^2} 
{m_{\tilde{f}_1}^2 -m_{\tilde{f}_2}^2 }
\end{equation}
and
\begin{equation}
m_{\tilde{f}_{1,2}}^2 = m_f^2 +\frac{1}{2} \left[
m_{LL}^2 +m_{RR}^2 \mp \sqrt{ (m_{LL}^2
-m_{RR}^2 )^2 +4 m_f^2 X_f^2 } \ \right]
\end{equation}
The mixing is very strong in the stop sector for large values of the parameter
$X_t=A_t- \mu \cot \beta$ and generates a mass splitting between the two mass 
eigenstates which makes the state $\tilde{t}_1$ much lighter
than the other squarks and possibly even lighter than the top quark itself.
These points shall be of interest later on, when we discuss the so-caleld 
``little hierarchy problem''.

\subsubsection{Gaugino and Higgsino sector}
The two charged Winos as well as the two charged Higgsinos can mix to yield four fermionic
mass eigenstates called charginos. These eigenstates have a tree-level mass matrix
\begin{equation}
{\cal M}_\pm =
  \begin{pmatrix}
    M_2 & \sqrt{2} M_W s_\beta \\
    \sqrt{2} M_W c_\beta & \mu
  \end{pmatrix},
\label{mchar}
\end{equation}
where $M_W$ is the $W$ boson mass and $s_\beta = \sin\beta$.

Next, the four gauge eigesntates $(\tilde{B},\tilde{W}^3,  \tilde{H}_u^0, \tilde{H}_d^0)$ can also
mix, giving rise to four mass eigenstates collectively called neutralinos. At tree-level, the neutralino
mass matrix is given by
\begin{equation}
{\cal M}_0 =
 \begin{pmatrix}
    M_1 & 0 & -M_Z s_W c_\beta & M_Z s_W s_\beta \\
    0 & M_2 & M_Z c_W c_\beta & -M_Z c_W s_\beta \\
    -M_Z s_W c_\beta & M_Z c_W c_\beta & 0 & -\mu \\
    M_Z s_W s_\beta & -M_Z c_W s_\beta & -\mu & 0
  \end{pmatrix}.
\label{mneutra}
\end{equation}\\
where $s_\beta = \sin\beta$, $c_\beta = \cos\beta$, $s_W = \sin\theta_W$,  $c_W = \cos\theta_W$,
$\theta_W$ is the Weinberg angle and $M_Z$ is the $Z$ boson mass.

The matrix \eqref{mneutra} is complex symmetric and can thus be diagonalized analytically 
by a unitary matrix $Z_0$ as
\begin{equation}
 {\cal M}_0 = Z_0 D_0 Z_0^\dag
\end{equation}
The exact form of $Z_0$ is, in the general case, quite complex. In the end, one gets
four mass eigenstates that we shall hereafter denote $\chi_i^0 \ ,  \ i = 1...4$.
\\ \\
Having presented the physical particle content of the MSSM, we can next wonder whether some
of these particles could account for the observed dark matter abundance.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Dark Matter in the MSSM}
So far, we have mainly focused on the completely minimal supersymmetric extension of the Standard Model.
In short, for every bosonic or fermionic degree of freedom in the SM, $N = 1$ global supersymmetry introduces 
a fermionic or bosonic one. Nevertheless, there are obviously numerous other extensions that can be envisaged,
depending on each author's concerns. In any case, whatever the precise model, it is reasonable to look for
candidates which are neutral under color and electromagnetism, as well as most probably stable (or at least
with couplings weak enough to prevent their rapid decay).

In the MSSM framework we presented, the imposition of $R$-parity renders the Lightest Supersymmetric
Particle completely stable. Potential candidates could be (referring to the physical states now) sneutrinos 
(left-handed, since we have not written down terms for right-handed neutrinos) or neutralinos. 
Furthermore, we note that once supersymmetry is rendered local, an additional candidate can
be found, the graviton's superpatner called gravitino. Gravitino dark matter has been studied
in a series of different frameworks, such as the MSSM \cite{Luo:2010he}, extensions of the former
that solve the so-called ``$\mu$ problem'' and/or the neutrino mass problem 
\cite{Choi:2009ng,Munoz:2009qp, Buchmuller:2007ui, Covi:2009xn, Covi:2009bk} and so on.
Then, one could aim at introducing right - handed
neutrinos in order to achieve a see-saw mechanism yielding small neutrino masses, in which case the
right-handed neutrino or sneutrino could enter the game (see, for example, \cite{Cerdeno:2008ep}). 
Finally, we should also mention that
in theories trying to address the absence of $CP$ violation in the strong sector via the introduction
of a Peccei - Quinn symmetry, the associated boson called axion is a plausible candidate. Although today
axions are rather constrained, if such a model is rendered supersymmetric, the axion's superpatner called
axino can provide a good candidate \cite{Covi:2004rb}.

Among these candidates, the most well - known and widely studied is the lightest neutralino
(often also called just neutralino).

\subsection{Neutralino dark matter}
We already mentioned that all neutralinos are linear combinations of the superpartners of the SM
neutral gauge bosons and the neutral higgs bosons. In a generic manner, we can write
\begin{equation}
 \chi_1^0 = Z_{11} \tilde{B} + Z_{12} \tilde{W}^3 + Z_{13} \tilde{H}_1^0 + Z_{14} \tilde{H}_2^0
\label{NeutralinoGeneric}
\end{equation}
where we assume that we have rearranged the neutralino matrix in order to have the lightest one
at the top row. Since neutralinos are comprised of four distinct contributions, all of which contribute
to the total couplings in different manners, it is customary to further define two quantities representing
the neutralino composition, namely the gaugino fraction and the higgsino fraction
\begin{eqnarray}
 f_G & = & Z_{11}^2 + Z_{12}^2\\ \nonumber
 f_H & = & Z_{13}^2 + Z_{14}^2
\end{eqnarray}
\\ \\
A huge amount of literature has been devoted to the study of neutralino dark matter. It is quite difficult
to present an overview of the relevant phenomenology in the case of the most general $R$ - parity conserving MSSM, 
since the number of free parameters in the general case is of the order of $120$, which is an uncontrollably
large parameter space to be probed efficiently.

The most usual approach towards supersymmetric phenomenology is to make simplifying assumptions, 
often (but not exclusively) motivated by some higher theory, aiming at the reduction of the number
of free parameters. One such example is the so-called Constrained MSSM (CMSSM). In this model, 
it is assumed that 
\begin{itemize}
 \item The three gauge couplings (properly normalized) meet at the Grand Unification Scale
 \item The Bino, Wino and gluino masses are universal at the GUT scale $M_1(\mgut) = M_2(\mgut) = M_3(\mgut) \equiv m_{1/2}$
 \item All scalar masses unify at the GUT scale
\begin{eqnarray}
m_{\tilde{Q}_i} (M_{U}) &=& m_{\tilde{u}_{Ri}} (M_{U}) =
m_{\tilde{d}_{Ri}}(M_{U})  =m_{\tilde{L}_i} (M_{U}) 
= m_{\tilde{\ell}_{Ri}} (M_{U}) \\ \nonumber
&=& m_{H_1}(M_{U}) =m_{H_2} (M_{U}) \equiv  m_0
\end{eqnarray}
 \item Trilinear couplings are universal at the GUT scale
\begin{equation}
A^u_{ij} (M_{U}) = A^d_{ij} (M_{U}) = A^\ell_{ij} (M_{U}) \equiv  A_0 \, 
\delta_{ij}
\end{equation}
\end{itemize}
If one further assumes a specific relation among the bilinear and trilinear soft breaking terms
as well as a relation between the gravitino and scalar masses, the resulting model is called
minimal supergravity (mSUGRA).

In the case of the CMSSM, the resulting model is described by only five free parameters:
$\tan\beta$, $m_{1/2}$, $m_0$, $A_0$ and $\mbox{sign}(\mu)$, where the last parameter is the
sign of the higgsino mass parameter. It can be demonstrated that demanding radiative electroweak 
symmetry breaking, minimization of the Higgs potential yields
\begin{eqnarray}
 B \mu & = & \frac{1}{2} 
\left[ 
(m_{H_1}^2 - m_{H_2}^2)\tan 2\beta + M_Z^2\sin 2\beta
\right]\\
 \mu^2 & = & 
\frac{m_{H_2}^2 \sin^2\beta - m_{H_1}^2 \cos^2\beta}{\cos2\beta}
- \frac{M_Z^2}{2}
\end{eqnarray}
which demonstrates that while the absolute value of $\mu$ is fixed, its sign remains
unknown.


In order to describe some typical features of neutralino
dark matter in the CMSSM, we borrow figure \ref{fig:CMSSMdark} from \cite{Ellis:2010kf}.
Non-dark matter - related constraints appearing in the figure are explained in the caption.

\begin{figure}[ht]
\begin{center}
\includegraphics[width = 8cm]{./susy/50pmap.eps}
\caption{{\footnotesize
$(m_{1/2}, m_0)$ plane for $\tan\beta = 50$, $\mu > 0$ and $A_0 = 0$. Red dot-dashed lines
correspond to $m_h = 114$ GeV and black dashed lines to $m_{\chi^\pm} = 104$ GeV. The brown 
region yields a stau LSP, the dark green region is excluded by $b \rightarrow s \gamma$ and
the pink region is favoured by the muon anomalous magnetic moment measurements. The turqoise
regions yield the correct relic density. Figure taken from \cite{Ellis:2010kf}
}}
\label{fig:CMSSMdark}
\end{center}
\end{figure}

We can clearly see from the figure that whereas the regions where the neutralino becomes the LSP
are quite significant,
the WMAP limits strongly restrict the viable parameter space. The WMAP - compliant regions
are represented in turquoise. It is interesting that despite 
the relatively small number of
surviving points, the processes contributing to getting the correct relic density vary from
one region to another. Let us start the description of these zones by stating that in most of
the parameter space, the CMSSM yields too large a relic density. The neutralino LSP is mostly
bino, and a bino LSP couples very weakly to both the $Z$ and the higgs bosons. The couplings
of the neutralino to various MSSM particles are presented in Appendix \ref{NeutralinoCouplings}.
Some enhancement is thus needed
in order to obtain WMAP-compliant results. For small $(m_{1/2}, m_0)$ values, the correct 
relic density is obtained through crossed-channel sfermion exchange. This is called the 
\textit{bulk region}. As $m_{1/2}$ increases, the correct relic density is obtained near the region
where the stau becomes the LSP. In this case, the dominant process
enhancing neutralino annihilation is actually its coannihilation with the lightest $\tilde{\tau}$, 
usually called the NLSP (Next-to LSP). This region is called the \textit{coannihilation region}. At larger
$(m_{1/2}, m_0)$ values and away from the coannihilation region, the self-annihilation cross-section
gets enhanced kinematically, since in this region two neutralinos can annihilate efficiently
into a nearly on-shell higgs propagator $H$ or $A$. This region is called the \textit{funnel region}.
Finally, there is a fourth region where the correct relic density can be obtained, called the
\textit{focus point/hyperbolic branch} region, where the neutralino obtains a significant higgsino fraction, 
resulting in an enhancement of its couplings to $Z$'s and higgs bosons. 
\\ \\
For the moment, we pause our discussion on neutralino dark matter in order to present an issue 
of the CMSSM related to the higgs boson mass, motivating the models that we shall be looking into
in the following.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{A parenthesis: the little hierarchy problem}
\label{LittleHierarchyProblem}
Starting from the discussion on the physical spectrum of the MSSM, it is quite straightforward to 
compute the model's tree-level prediction for the neutral $CP$ - even higgs boson masses.
The result is
\begin{equation}
 m_{h, H}^2 = \frac{1}{2} 
\left[
m_Z^2 + m_A^2 \mp 
\sqrt{(m_A^2 - m_Z^2)^2 + 4 m_A^2 m_Z^2 \sin^2 2 \beta}
\right]
\label{TreeHiggs}
\end{equation}
From this equation we can see an immediate problem: denoting the lightest of the
two higgses by $h$, we see that its mass is forcedly lower than the $Z$ boson mass.
LEP2 has posed the most stringent existing bounds on the lightest higgs boson mass
for the Standard Model \cite{Barate:2003sz} and the MSSM \cite{Schael:2006cr}. In the former case, this
limit is very stringent $m_h > 114.4$ GeV. In the MSSM case, the situation turns out
to be slightly more complicated.

These bounds come mainly from two direct search channels, namely higgsstrahlung and associated 
production of $h$ and $A$. For later use, we note that the cross-sections for these processes
are, in comparison to the Standard Model higgsstrahlung case
\begin{eqnarray}
 \sigma(e^+ e^- \rightarrow hZ) & = & g^2_{hZZ} \sigma_{\mbox{\begin{tiny}SM\end{tiny}}}(e^+ e^- \rightarrow hZ)\\ \nonumber
 \sigma(e^+ e^- \rightarrow hA) & = & g^2_{hAZ} \sigma_{\mbox{\begin{tiny}SM\end{tiny}}}(e^+ e^- \rightarrow hZ) \times
\frac{\lambda_{Ah}^2}{\lambda_{Zh} (\lambda_{Zh}^2 + 12 M_Z^2/s)}
\label{HiggsProdLEP}
\end{eqnarray}
where $m_Z$ is the $Z$ boson mass, $s$ is the center-of-mass energy of the collision, 
$\sigma_{\mbox{\begin{tiny}SM\end{tiny}}}(e^+ e^- \rightarrow hZ)$ is the higgsstrahlung 
cross-section in the SM, $\lambda_{ij} = (1 - M_i^2/s - M_j^2/s)^2 - 4 M_i^2 M_j^2/s^2$ and
the two couplings $g_{ijk}$ are given by the higgs mixing angles
\begin{eqnarray}
 g^2_{hZZ} & = & \sin^2(\beta - \alpha)\\ \nonumber
 g^2_{hAZ} & = & \cos^2(\beta - \alpha)\\ \nonumber
\end{eqnarray}
The LEP2 bound $m_h \gtrsim 114$ GeV is actually also applicable to the MSSM, in the 
case where $g^2_{hZZ} = {\cal{O}}(1)$.
\\ \\
In fig.\ref{fig:LEPHiggsBSM}, taken from \cite{Schael:2006cr}, the LEP collaboration 
calculates the limits on the squared ratio
$\xi^2 = (\sigma_{hZZ}/\sigma_{hZZ}^{SM})^2$ between a generic BSM $hZZ$ coupling and
the Standard Model one as a function of the higgs boson mass. As we can see from
the figure, once the squared coupling becomes smaller than $1$, there is indeed much 
space for lighter $h$ masses. Refering to eq.\eqref{HiggsProdLEP}, the $\xi$ factor
would be simply $\sin(\beta - \alpha)$.

\begin{figure}[htb]
\vspace{2cm}
\begin{center}
\includegraphics[width = 10cm]{./susy/LEPHiggsBSM.eps}
\caption{{\footnotesize
$95\%$ CL upper bound on the ratio $\xi^2 = (g_{hZZ}/g_{hZZ}^{SM})^2$.
Figure taken from \cite{Schael:2006cr}.
}}
\label{fig:LEPHiggsBSM}
\end{center}
\end{figure}

The problem in CMSSM and mSUGRA-like models arises from the fact that in these models the suppression
factor is typically ${\cal{O}}(1)$. An example analysis is presented in \cite{Kane:2004tk}, 
where it can be seen that a Light Higgs Scenario (LHS) cannot be realized within the 
framework of mSUGRA without introducing tensions with other observables.
\\ \\
One the other hand, eq.\eqref{TreeHiggs} is a tree-level prediction.
Once one starts taking seriously into account the quantum nature
of the MSSM and includes radiative corrections to the higgs mass, these turn out to be quite sizeable
for some regions of the CMSSM parameter space. However,
even in this way, there are some requirements which often appear to be quite restrictive \cite{Djouadi:2005gj}:
\begin{itemize}
 \item From eq.\eqref{TreeHiggs} we can see that the large $\tan\beta$ regime is rather favoured, 
since then the lightest higgs mass approaches its highest tree-level limit, the $Z$ mass.
 \item Even after the inclusion of radiative corrections, it turns out that the regions of the
parameter space where the LEP2 limits can be satisfied are somewhat restricted, requiring either
large stop masses (the stop sector gives the dominant contribution to the higgs mass), either
substantial left-right stop mixing.
\end{itemize}

We thus see that in order to obtain a large enough Higgs mass, quite particular assumptions must be
made concerning the values of $\tan\beta$, the masses and mixings of the stop sector, or the
relation among the two higgs mixing angles.
Furthermore, assuming large stop masses starts posing once again issues with the hierarchy 
problem, since we already mentioned that the superpatner masses should be as close to the
electroweak scale as possible in order to efficiently cancel the higgs mass quadratic divergencies.
This problem is referred to as the \textit{little hierarchy problem}.
\\ \\
According to this discussion, two possible wayouts could be envisaged:
\begin{itemize}
 \item Taking into account contributions to the Higgs mass that could come from
physics beyond the MSSM (BMSSM), which are known to be persent in several of its
extensions.
 \item Trying to find a framework which does not necessarily modify the particle
content of the MSSM, but instead focuses on reducing $\sin(\beta - \alpha)$.
\end{itemize}
In the remaining of this work we shall be examining dark matter in two supersymmetric 
frameworks trying to evade the little hierarchy problem in both ways.














